Moving Beyond LDA: A Comparison of Unsupervised Topic Modelling Techniques for Qualitative Data Analysis of Online Communities

Social media constitutes a rich and influential source of information for qualitative researchers. Although computational techniques like topic modelling assist with managing the volume and diversity of social media content, qualitative researcher's lack of programming expertise creates a significant barrier to their adoption. In this paper we explore how BERTopic, an advanced Large Language Model (LLM)-based topic modelling technique, can support qualitative data analysis of social media. We conducted interviews and hands-on evaluations in which qualitative researchers compared topics from three modelling techniques: LDA, NMF, and BERTopic. BERTopic was favoured by 8 of 12 participants for its ability to provide detailed, coherent clusters for deeper understanding and actionable insights. Participants also prioritised topic relevance, logical organisation, and the capacity to reveal unexpected relationships within the data. Our findings underscore the potential of LLM-based techniques for supporting qualitative analysis.

==> chapter-pilot.tex <==
%======================================================================
\section{Pilot Study}
%======================================================================

We conducted a pilot study to assess and refine our research design, topic modelling techniques, and to gather feedback on the study's structure. By involving Human-Computer Interaction (HCI) researchers with diverse expertise, we sought to gain valuable insights and perspectives to improve our methodology and address any challenges that might arise during the main study. 

We chose the \textbf{r/uwaterloo} subreddit as our primary data source because of its lively and engaged community, which is relevant to the study's themes and our test group of HCI experts from the university. Data collection was facilitated through web scraping techniques implemented using custom scripts discussed in \autoref{data_collect}. We sampled data from January 1st to December 31st, 2023 (01/01/2023 - 31/12/2023). The collected data, comprising comments and submissions, amounted to 15,793 documents.

        
\section{Participants}

Ten HCI researchers participated in the study, including four professors, one postdoctoral researcher, and five master's students. The were experts in thematic analysis, user experience (UX) research, and immersive technologies like gaming and virtual reality. All participants were fluent in English.

       
  
\section{Procedure}
We delivered a 10-minute presentation, encouraging participants to ask questions and provide feedback. Following this, we provided each participant with a printed copy of the Microsoft Desirability Toolkit \citep{benedek2010measuring, rohrer2008desirability} and a set of interview questions (\autoref{tab:interview_phase2}). We also provided participants with printed copies of topics and keywords generated by each topic modelling algorithm --- LDA, Top2Vec, and BERTopic. A full copy of the topics and keywords are available in \autoref{materials}.
        
After participants completed the analysis and responded to the interview questions, the session transitioned into an open discussion format. During this interactive segment, participants were encouraged to share their insights, provide feedback, articulate their comments, and elucidate their rationale behind selecting a specific model. Additionally, participants engaged in group discussions surrounding the criteria for ranking the models, considering factors such as their comprehension, familiarity, and acceptance of the results. 


\section{Data Collection and Analysis}
       
We generated topic models using three unsupervised topic modelling algorithms: LDA, Top2Vec, and BERTopic. We then transcribed topic keywords generated by each algorithm into a tabular format for qualitative and analytical interpretation by participants (\autoref{fig:lda_pilot}, \autoref{fig:top2vec_pilot}, \autoref{fig:bertopic_pilot}).


\begin{figure}[p]
    \centering
   \fbox{ \includegraphics[width=1\textwidth]{images/lda_pilot.png}}
    \caption[Pilot study results for LDA]{LDA topics and keywords, \texttt{topic\_id} depicts the topic number, the \texttt{topic\_keywords} describe the keywords generated by the model, and the other quantitative results show the characteristics for this specific topic in the corpora.}
    \label{fig:lda_pilot}
\end{figure}


\begin{figure}[p]
    \centering
    \includegraphics[width=1\textwidth]{images/top2vec_pilot.png}
    \caption[Pilot study results for Top2Vec]{Top2Vec topics and keywords, ${\pi}$ depicts the topic number, the \texttt{keywords} describe the keywords generated by the model, by default it gives the first 50 words asscociated with the model.}
    \label{fig:top2vec_pilot}
\end{figure}

\begin{figure}[p]
    \centering
   \fbox{\includegraphics[width=0.6\textwidth]{images/bertopic_pilot.png}}
    \caption[Pilot study results for BERTopic]{BERTopic topics and keywords, \texttt{Topic 6} depicts the topic number, the string words describe the keywords generated by the model, and the numeric values depict the probability of the keyword, by default it gives the first 10 words asscociated with the model.}
    \label{fig:bertopic_pilot}
\end{figure}

       
    
    % We began the data collection process with each participant analyzing the outcomes derived from the three distinct topic modelling algorithms. Following this analysis, participants provided their insights and responded to a series of questions outlined in the second phase of the interview protocol, in \autoref{tab:interview_phase2}. This phase, conducted after participants explored the results from the three different topic models, we aimed to gather detailed feedback on its efficacy and relevance. Participants used the Microsoft Desirability Toolkit to describe our method and ranked the LDA, Top2Vec, and BERTopic models based on usefulness, explaining their rankings. We compared our method to existing tools, explored model relevance to their research, and discussed integration challenges. Participants rated the likelihood of incorporating our model into their work on a scale of 1-10 and provided additional insights. This phase aimed to understand the practical utility and potential improvements for our approach.

We began data collection by asking participants to inspect each of the three topic models. They then moved to questions from the second phase of the interview protocol (\autoref{tab:interview_phase2}). Participants used the Microsoft Desirability Toolkit to describe each topic model. They compared the models to existing tools they currently use, discussed integration challenges they might face while incorporating them into their research, their practical utility, and potential improvements.
    
The data analysis phase involved two distinct components: a quantitative analysis that focused on the evaluation metrics (topic coherence, topic diversity and execution time) results and a qualitative examination that involved gathering subjective feedback from the participants. Each participant's feedback was carefully reviewed, and a comprehensive summary document was compiled to highlight the key points and observations shared by the participants. Although the primary focus of the pilot study was on qualitative insights, the quantitative findings provided supplementary information that aligned with our overarching objectives.

   

\section{Quantitative Results }


Our quantitative analysis revealed that BERTopic achieved the highest performance in terms of topic coherence, followed by LDA, with Top2Vec demonstrating the lowest topic coherence. Regarding topic diversity, both BERTopic and LDA outperformed Top2Vec. However, in terms of runtime and execution, LDA was the fastest, followed by Top2Vec, with BERTopic taking the longest time. These findings are summarized in \autoref{tab:model_performance}. 




\begin{table}[tb!]
    \centering
    \scriptsize
    \caption{Summary of Model Performance: Pilot study}
    \label{tab:model_performance}
    \begin{tabular}{ p{3cm} p{3cm} p{3cm} p{3cm} }
        \toprule
        \textbf{Model} & \textbf{Topic Coherence} & \textbf{Topic Diversity} & \textbf{Run Time (seconds)} \\ 
        \midrule
        BERTopic & 0.62 & 1 & 270 \\ 
        LDA & 0.56 & 1 & 25 \\
        Top2Vec & 0.36 & 0.67 & 258 \\ 
        \bottomrule
    \end{tabular}
   
\end{table}

 
\section{Qualitative Results }

Participants' feedback highlighted key differences among the three topic modelling algorithms. BERTopic was ranked first by 5 out of 10 participants (50\%), Top2Vec by 3 out of 10 participants (30\%), and LDA by 2 out of 10 participants (20\%). BERTopic was the most favoured, with five participants ranking it highest for its comprehensive results, intuitive presentation, and logical grouping of topics, despite some finding the probability numbers complex. Top2Vec received mixed feedback; some appreciated its representational capabilities, while others found it challenging due to the lack of numerical values. LDA garnered the least enthusiasm, with topics seen as irrelevant and confusing. However, a few participants appreciated its qualitative and quantitative comparison. Notably, one participant switched their preference from LDA to BERTopic after discussions, highlighting the impact of collaborative discussion. 

%Overall, the study emphasized the importance of user perspectives in evaluating topic modelling algorithms, guiding future protocols for the main user studies.


      
%  \begin{table}
  
%     \centering
%     \scriptsize
%      \caption{Comparison of Attributes Across Models: Microsoft Desirability Toolkit}
%     \label{tab:model_comparison}
%      \begin{tabular}{ p{3cm} p{3cm} p{3cm} p{3cm} }
%       \toprule
%         \textbf{BERTopic} & \textbf{Top2Vec} & \textbf{LDA} \\
%        \midrule
%         Accessible & Understandable & Understandable \\
%         Clean & Accessible & Clean \\
%         Organized & Relevant & Incomprehensible \\
%         Reliable & Organized & Inconsistent \\
%         Consistent & Familiar & Undesirable \\
%         Understandable & Expected & Ineffective \\
%         Meaningful & Simplistic & Overwhelming \\
%         Satisfying & Entertaining & Irrelevant \\
%         Relevant & Usable & Not Valuable \\
%         Expected & Inconsistent & Poor quality \\
%         Useful & Intuitive & Incomprehensible \\
%         Predictable & Hard to Use & Confusing \\
%         Convenient & Inconsistent & Difficult \\
%         Overwhelming & Intimidating & Unrefined \\
%         Rigid & Overwhelming & Hard to Use \\
%         Disconnected & Busy & Unattractive \\
%         & Time-consuming  & \\
%         & Unattractive & \\
%         &  Unrefined & \\
%           \bottomrule
%     \end{tabular}
     
% \end{table}


    
\section{Discussion}
   
%Based on the insights gathered from the pilot study, it is evident that each model, BERTopic, Top2Vec, and LDA, offers unique advantages and limitations. 

BERTopic emerged as the preferred choice among participants, who commended it for its comprehensive and easily interpretable results. Participants appreciated its semantic grouping of topics, clear ranking presentation, and its probability information. Furthermore, these results align with our quantitative analysis, which demonstrated that BERTopic outperformed both LDA and Top2Vec in terms of topic coherence and semantic grouping. In terms of topic diversity, BERTopic and LDA surpassed Top2Vec. 

However, after conducting the pilot study we recognized the need for methodological adjustments. First, given the similarities between BERTopic and Top2Vec, we decided to replace Top2Vec with Non-Negative Matrix Factorization (NMF). NMF was chosen for its matrix-based approach, which differs from the probabilistic methods of LDA and neural-network methods of BERTopic. 

Participant feedback also emphasized the need for more consistent visualization of topic models. Participants struggled to compare topics between the different models, and inconsistent formatting and use of weightings in the printed copies prompted participants to focus on superficial differences. To address this issue we decided to incorporate BERTopic into the Computational Thematic Analysis toolkit so that all models could be compared within a single, consistent, and interactive interface. 

Finally, we found that participants were more articulate when speaking about the models rather than when writing. Consequently, we structured our user studies as semi-structured interviews, allowing us to transcribe their responses for analysis. Having addressed these issues, we decided to extend our research to include a broader sample of researchers and datasets. 

%This expansion was crucial to validate the initial findings and ensure that BERTopic's performance was generalizable across diverse research areas and larger datasets.

%Moving forward, the insights gained from this study informed the selection and implementation of topic modelling techniques and interview procedures for our main user case study.

      
        



==> extras.tex <==
%======================================================================

%======================================================================
\subsection{LDA}
Researchers provided mixed feedback on the LDA (Latent Dirichlet Allocation) model, appreciating its simplicity and ease of use while acknowledging its limitations in detail and relevance. A few participants preferred LDA for its familiarity and straightforward results, stating it as their top choice due to ease of access and clarity. LDA was valued for producing clear, organized outputs, making it accessible for those seeking quick and easy-to-understand results. However, its lack of depth and tendency to generate broad or sometimes irrelevant topics were noted drawbacks.

Some participants perceived LDA as relevant, accessible, and clear. P3 highlighted its relevance and ease of use, stating, ``[For] LDA [I put] `relevant' because I think those topics feel relevant and easy to combine into higher level themes. It's very easy to find information about LDA online and it's pretty easy to learn it.'' P11 appreciated the meaningful groupings created by LDA, noting, ``This model has created groupings that are more meaningful than NMF. There is a common thread across the keywords and there wasn't any random noise blocking the signal of understanding."  They also mentioned the advantage of LDA producing fewer topics, making it easier to focus on each one equally: ``The LDA had the least amount of topics, so it was easier from a user design perspective to pay attention to all of them equally as opposed to the third model [BERTopic] like 56.'' 


However, other participants noted limitations of LDA, primarily highlighting issues of disconnection, lack of meaningful clusters, and confusion in the result from their datasets. For instance, P2 pointed out that the topics generated by LDA were not semantically meaningful and often felt disconnected: ``The topics themselves are not really like semantically meaningful. I wouldn't go as far as calling them incomprehensible, but I think if there's just like a word like meaningless, that would describe it.''  P6 felt that LDA lacked depth in its topics, making it hard to understand the connections between them:
``LDA tells you about hey, this is sustainable fashion, but that's it. I'm not getting anything more. It's not telling me how are they connected? What's the conversation that's taking place? Say, Topic 15 [Topic keywords: \textit{sustainable, esg, sustainability, blog, long, impact, fit, time, wear, fashion}] talks about ESG, but then that's it. So, but then it's talking about sustainability. How is it relevant? What's happening? What's the conversation that's taking place? So that's what at it's making it a bit confusing and not valuable to me.  Some of the words that clusters don't make sense. Like topic six [Topic keywords: \textit{user, textiles, flip, \&, cork, flops, new, old}], it has flip flops [and] textiles. I'm not sure how they're relevant.'' On a similar note, P7 noted the presence of irrelevant content and rogue keywords, leading to a lack of clarity and predictability:
``There was a lot of irrelevant content there. LDA was also a bit old. There were a bunch of clusters in LDA where it had rogue keywords. So I wouldn't call it understandable. Unpredictable, I think.'' P8 described LDA as disconnected, not valuable, and rigid, with topics that seemed arbitrarily thrown together:
``Numerous clustering words could have been in any of the other clusters. It just felt like it was thrown together. So I didn't think it was flexible and it wouldn't be desirable for my area. Because my area is more getting to the specifics. Well, why would, increased water intake, improve diet quality [Topic keywords: \textit{sugar, water, like, milk, drink, people, fruit, salt, food, good}]? Why would plant based protein intake improve diet quality more aligned with the Canada Food Guide? It [clusters] didn't relate to me.''

While the default settings effectively removed most symbols, they were not flawless, affecting all topic models to some extent. This issue appeared to be most pronounced with LDA. For instance, P2 indicated that LDA often grouped irrelevant symbols and mathematical characters together, detracting from meaningful clustering: ``They have a topic for just mathematical characters like equal sign and these are all like either code or Math quantifiers or symbols [Topic keywords:  \textit{=, \#, message, compose/?to, import, r, \,; def, +}]. This one has literally an asterisk [Topic keywords: \textit{model, \&, models, * language, code, paper, training, tokens, -}]. And also like just looking at these, not a lot of them really seem like clusters.'' 
Another observation from P10 found LDA unrefined, noting the presence of irrelevant symbols and lack of meaningful topics:
``The thing that bugs me the most is like I see sometimes there's emojis. Sometimes there's just like a hyphen or just a space [Topic keywords: \textit{co, -, op, coop, work, program, job, waterloo, cs, like}]. 





\subsection{NMF}

The NMF model technique was valued for producing clear, relevant, and organized topics, making it a reliable choice for research. The model generated clean, usable clusters with an organized structure. However, it was sometimes too general, missing nuanced details that other advanced models captured. Overall, NMF balanced detail and usability, offering clear and relevant outputs that were easy to interpret, but it fell short in capturing the full complexity of certain topics.

Participants valued NMF for its relevance and clear organization, which made it straightforward and usable for understanding current trends. P2 appreciated the succinctness and statistical relevance of NMF.  
P5 found NMF more relevant in terms of the actual keywords and topics from Reddit:
``When I use the NMF, it was more relevant. I found more relevancy in terms of the actual keywords used in the topic model and also the actual Reddit. Quickly having an overview, I found it [had] more relevant keywords.'' P6 highlighted NMF's clarity and organization, making it easy to understand current trends:
``It looks clean to me. The clusters make sense, and they're relevant to the current scene. It's organized and usable because, based on the clusters, I can understand the current trend. It's very straightforward.'' P8 also found NMF consistent, approachable, and useful and stated:
``I thought this model was better than the first one [LDA]. The clustering of names was more similar and made sense together, so it was consistent. It was inviting because it was simplistic and approachable.''  P1, P2 and P11 felt NMF was simplistic and efficient since the number of topics were less: (P1) `` but this is easier to read because there's less [content]", (P2) ``Fewer topics, I think is always better" and  
(P11) ``For this one, it's simplistic and essential, but also efficient. The topics are kept small, and the results are pretty expected.'' 

Researchers identified several limitations with NMF, noting its generality, topic overlap, and lack of semantic clarity. P1 mentioned that the number of topics was insufficient for a large dataset:
``This isn't enough. So I think [number of topics as] 5 is definitely not enough for such a large data set in my opinion." P2 criticized its lack of semantic meaning:
``They are not semantically meaningful or relevant. It needs a lot more refining at a semantic level.'' P2 also felt that while NMF produced fewer topics, they were too broad and not necessarily more meaningful:
`` Yeah, this is extremely coarsely grained. It's just way too broad. It seems to be more decisive than LDA, but it's not really anymore meaningful.'' P3 pointed out the overlap between topics and suggested combining them:
``There's overlap between topics, but I don't mind that. I would just combine them.''
 P7 noted some undesirable keywords and rigidity:`` There were a few clusters with undesirable keywords like cluster three [Topic keywords: \textit{message, compose/?to, \#, import, \&, remindmebot\&amp;subject, ; amp;\#x200b, r]} It could not capture some topics, so it's a bit rigid in its organization. Some of these clusters maybe we did not need those clusters.''
P8 found NMF too general and lacking specificity:
``NMF is kind of a bit too general. You can say that[some topics] for any university.'' P9 noted that NMF did not capture keywords from other languages as compared to LDA and BERTopic for the r/Coronavirus data. P11 described NMF as unrefined, confusing, time-consuming, and difficult:
``Compared to the other two, this one was not pulling together themes relevant to the topic.''
  

\textbf{Summary of Findings for NMF}: 




\subsection{BERTopic}

BERTopic was highly praised for its comprehensive coverage, detailed analysis, and intuitive clustering, making it valuable for qualitative research across diverse subjects. Researchers appreciated its ability to generate detailed and relevant topics, providing fine-grained and meaningful insights. The model's attention to subtopics, such as sustainable fashion and AI trends, offered valuable, specific insights. The intuitive and coherent clustering made data easier to understand and interpret, with well-organized keywords that made sense. This specificity helped researchers focus on relevant topics without being overwhelmed. However, some researchers found BERTopic initially overwhelming due to the large number of topics and its complexity. This made navigating and digesting the information challenging at first.
Overall, BERTopic balanced comprehensive coverage with detailed analysis, offering valuable insights that were easy to interpret despite initial complexity. This made it a preferred choice of almost 83\% participants.


Participants consistently highlighted BERTopic's strengths in producing detailed, organized, and coherent topic clusters. Its usability was praised, with users noting that BERTopic provided more detailed and organized topics compared to other models. P1 noted, "BERTopic had more detailed and organized topics that are usable." Despite initial complexity, it was found to be superior in detail, offering high-quality and coherent keywords and clusters that were easy to view both visually and through direct data connections. P12 emphasized the coherence of its keywords and clusters, mentioning, "The ease of use and the ability to view it both visually and connecting right into the actual data." BERTopic's clear separation and specificity were highly valued, making it easy for users to recognize relevant terms. This distinctiveness helped in identifying and understanding related terms and their connections. P6 commended BERTopic for its sophisticated clusters, providing deep insights into specific subjects like vegan leather and ESG investments. For instance, "Topic 7 [Topic Keywords: \textit{leather, vegan, veganism, plant, plastic, animal, based, products, diet, meat}] discusses leather but delves deeply into vegan leather and plastic." Similarly, "The ESG cluster [Topic Keywords: \textit{esg, blog, investing, inrate, impact, governance, risk, investors, ratings, engagement}] informs me about investment. I can see the word governance and understand the impact," which contrasted with the LDA model, which struggled to link related concepts like ESG and sustainability effectively. P3 found the connections made by BERTopic intriguing and effective for their use case. Initially skeptical about the relevance of certain keywords, they realized through analysis that the model made meaningful connections. For example, P3 noted, "It's very interesting. When I was doing the analysis, I would not have connected horses and dewormer and Apple ivermectin [Context: Farm supply stores told CBC News they received an influx of calls from people looking to buy the livestock dewormer ivermectin, due to false claims that the apple-flavoured paste will cure or prevent COVID-19], [Topic keywords: \textit{horse, paste, horses, dewormer, apple, neigh, flavored, equine, glue, ivermectin}]." This highlighted BERTopic's ability to reveal unexpected but significant relationships within the data. 

P7 found BERTopic highly effective and easy to understand, noting its coherent grouping of related keywords:
``It's definitely helpful. It's definitely effective. It's easy to understand... Everything speech-related is in one cluster. [Topic Keywords: \textit{speech, audio, voice, whisper, recognition, asr, transcription, file, transcribe, text}] Overall, I see much more coherence here. The keywords make much more sense than the other two algorithms. I'm seeing much fewer rogue keywords."
P7 also valued BERTopic's inclusion of contemporary topics like prompt engineering [Topic Keywords: \textit{prompt, engineering, llms, comprehensive, curated, guide, resource, hand, promptslab, aws}]:
``I did not see anything about prompt engineering in the other algorithms, even though it's common these days."

% \textbf{User Experience and Practicality}:
P8 described BERTopic as appealing, effective, personal, and satisfying. They appreciated its ability to group related topics clearly:
``It is complex because there are many windows and connections, but appealing because it lumps similar topics together. This makes it easier to ignore irrelevant topics and focus on what's important to my work."

P8 found BERTopic more specific than other models, reducing the need to examine every individual topic:
``This specificity means I don't have to go into each and every topic. If it doesn't relate to my area, I can easily eliminate it. For example, topics like 26 or 15 that don't relate to my area can be ignored, making it simpler and more personal."

P9 found BERTopic more helpful and relevant than other models:
``It is more relevant, understandable, and valuable."

P10 praised BERTopic for the quality and consistency of its keywords, as well as the relevance and specificity of its topics. They found that the model effectively summarized subreddits and captured unique aspects of specific cultures:
``Mainly just the quality, like the consistency of the keywords as well as the number of topics and if I felt like the topics could summarize the subreddit. Pointing to the [Topic keywords: \textit{pd, pd11, fuck, pd1, course, pds, report, pd8, pass, pd5}], that's something specific to like Waterloo and Waterloo Coop. It's funny how this method found something that's uniquely part of Waterloo culture."

P10 also appreciated how BERTopic identified keywords specific to local restaurants:
``For example, Topic 38 [Topic keywords: \textit{lazeez, sauce, shawarma, lines, hot, eat, garlic, eating, lazeeza, diarrhea}] relates to Lazeez, which is popular on our Waterloo Campus Plaza."

P11 highlighted the model's ability to cluster terms related to specific conditions and therapies, providing detailed insights into subtopics:
``One of the subtypes of condition, PTSD, is post-traumatic stress disorder. BPD is for borderline personality disorder [Topic keywords: \textit{bd, bp, bp2, ptsd, mbti, onset, cps, pd, awakening}]."

%related to research 
% \textbf{Relevance to research}: 
Researchers consistently highlighted the relevance and nuanced approach of BERTopic, making it highly useful for their specific research contexts.
P12 found BERTopic's approach aligned with their literature review and research on social media communication: ``It definitely aligns with the literature review and research that I've gathered related to information on social media. I've been looking at alternative communication channels and how those channels are very active, even though official news media or government official channels have been sort of quiet [Topic keywords: \textit{reliable, political, institution, linking, submission, recognized, source, dedicated, submit, organization}]." 

P6 also found BERTopic's relevance to their research on sustainable fashion particularly noteworthy: ``It's really relevant and so it's very interesting that ESG's topic is coming out when we're talking about sustainable fashion. And then, OK, so this is circular economy, this is what my research is about, [Topic Keywords: \textit{circular, kindly, economy, survey, understanding...shion, adoption, research, advance, description}]. So it's very interesting to see it here as a part of the conversation when it comes to the sustainable fashion." P6 appreciated how BERTopic's nuanced approach enhanced their research: ``I'm already coming into the research with specific ideas and specific coding that I'm gonna use, but sometimes it's also good to look into what others and how others interpret the same material. So it would be interesting to use this module to see how it interprets my reporting and the websites of the companies that I'm looking into. And yeah, and just kind of give me a very nuanced understanding of the problem, which is what's really needed when it comes to qualitative research. You really want to look into the nuances and just examine them in that sense." 

On a similar note, P2 highlighted BERTopic's effectiveness in parsing and differentiating different topics, making it highly relevant and useful for their research: ``For my own research work, just because it seems to be pretty good at parsing and differentiating different topics and I can trust it, the other [models] seem to be statistically doing something but not nearly enough to make it useful. In research, I don't really care how much time I have to spend, but I wanna make sure what I write down on my papers or what I take from a paper has to be relevant. It has to be true."
 

Researchers consistently praised BERTopic for its comprehensive coverage, detailed analysis, and intuitive clustering, making it a valuable tool for qualitative research across diverse subjects.

% \textbf{Broad Coverage and Detailed Analysis:} 
P1 emphasized the importance of BERTopic's ability to cover a broad range of topics, particularly in qualitative research involving diverse subjects such as disability. They noted that the model's comprehensive nature allows for capturing meaningful insights, even from single mentions. P1 highlighted, ``It had the most detail out of all the models and gave the biggest range of topics,'' making it the best among the models evaluated.

% \textbf{Meaningfulness and Trustworthiness:} 
P2 found BERTopic to be meaningful, trustworthy, and comprehensive. They appreciated the model's ability to generate detailed and relevant topics with clear relationships between words, making the clusters semantically relevant and fine-grained. P2 noted, ``I think they're trustworthy because they have a lot of words that are very clearly related to each other. So for me, that builds trust. There's no question that there are a lot of topics, and they definitely cover just about every topic a human would identify.'' Additionally, P2 valued BERTopic's effectiveness in identifying trending topics in AI, such as llama-based chat GPT variants, reflecting current research interests: ``These are all talking about specifically llama and you know llama dot CPP and all of these like Llama-based chat GPT variants [Topic keywords:  \textit{llama, llama2, cpp, mayonnaise, ms, xethub, ggml, file, run, mount}]. So that's quite fine-grained and nice to see.''

% \textbf{Importance of Subtopics in Specific Fields:} 
P6 appreciated BERTopic's detailed coverage of subtopics within sustainable fashion, such as fabrications and dyes. They highlighted the model's attention to environmentally friendly dyes and health-related topics, which are significant in the industry but often overlooked. P6 noted, ``Fabrications and dyes are very important topics within the sustainable fashion world because some dyes are more environmentally friendly, and historically, some dyes caused health issues for fashion workers. This is a very important topic that I believe the industry is not really talking a lot about, but it's very interesting to see it here.''

% \textbf{Intuitive and Coherent Clustering:} 
P7 emphasized the intuitive and coherent clustering of BERTopic, which made the data easier to understand and interpret. They noted that the model's fine-grained clusters helped avoid the overlap seen in other models, making the results more accessible and logical. P7 stated, ``The clusters here are more fine-grained and easier to understand. When I make these plots, clusters often overlap, making it hard to understand why the model grouped certain data points together. But with BERTopic, the clustering was intuitive and made sense.''

% \textbf{Specificity and Logical Grouping:} 
P8 and P12 appreciated BERTopic's specificity and logical grouping of keywords. P8 noted, ``It gets a little bit more specific, which I like. It narrowed the topics down to numerous categories instead of lumping them together, making more sense in terms of what was clustered together.'' P12 highlighted the logical organization of 62 topics, finding the clustering intuitive and easy to comprehend: ``I like how the keywords are captured into 62 topics – and they seem to make more sense as groupings. I don't know if I would need all 62 topics, but I like that they've broken it out that way because a lot of the language clustered together makes sense. Just glancing through, the way they've clustered the words makes more sense to me. [Topic keywords: \textit{mask, masks, wear, wearing, people, face, n95, like, public, use}]''


While some praised BERTopic's detailed and organized approach, others found it overwhelming and challenging to navigate. Key themes that emerged from their feedback include concerns about transparency and clarity in data grouping, the model's complexity, and its overall usability.
For instance, P1 expressed concerns about the transparency and clarity of BERTopic's data grouping:
``I can't make that assumption unless I see the data, and right now I can't see the data. We wanna actually see the data, but it's also I'm curious why they would group blind and deaf together. Understanding accessibility needs for blind versus deaf are very different because they have different needs and pain points. I don't understand why some of these things are grouped together. I'm sure there's a valid reason, but I just need to know the why and I don't see the why in this."

P2 found BERTopic slightly overwhelming but appreciated its efficiency in conveying information:
``I feel like it could be more succinct, like there is room for improvement, but generally I really couldn't complain because as a human, I can just choose to read one or two words. It's really quick for me to look at even however many words there are. I can pretty quickly get a sense of what the cluster is about, so I don't even consider this."

P3 found BERTopic overwhelming and overbearing due to the sheer number of topics, despite acknowledging their meaningfulness and relevance:
``I'm going to say overwhelming as my first one. It is meaningful and a lot of the topics are interesting and relevant, but it is overwhelming and overbearing because I don't think all of those topics are necessary. It's distracting and unrefined." They ranked BERTopic last compared to LDA and NMF due to its complexity:
``I would rank LDA first because I know it and I'm most familiar with it. NMF would be second because it gives me fairly familiar results. I would rank BERTopic last because it is so massive, and while the topics fit better, there are way too many topics. It's just too much."

P4 also found BERTopic challenging to navigate:
``When I clicked the BERTopic diagram, it was very hard to click, but it's very easy to click LDA by the topic because there is some space between the topics and I can see more clearly." P11 described BERTopic as unconventional, complex, and busy, though still easy to use once understood:
``Yeah, this one is a bit overwhelming. I wrote unconventional, complex, and busy. It was a bit unrefined due to the sheer amount of content and unnecessary web links in the keywords. There was a lot going on, making it hard to digest the key points."

  
\chapter{Data Analysis and Preparation}

\section{Introduction}

%The success of any research project hinges on the meticulous preparation and analysis of data. In this chapter, we delve into the processes undertaken to prepare and analyze the data collected for this study. The primary objective is to ensure that the data is clean, well-structured, and suitable for subsequent analysis phases.

This study involved conducting twelve interviews with qualitative researchers. During these discussions, we leveraged their expertise to collaboratively finalize datasets that were suitable for the research objectives. These datasets were sourced from Reddit, ensuring a diverse and relevant data pool aligned with each researcher's domain. These datasets span a diverse range of domains, including gaming, technology, COVID-19, health, environment, politics, and one dataset specific to the University of Waterloo. Each dataset presents unique characteristics and challenges, necessitating a comprehensive approach to data preprocessing and transformation. 











\section{Data Collection}



%In this section, we detail the comprehensive procedures undertaken for data collection. The data utilized in this study was sourced from Academic Torrents, which includes extensive subreddit data up to December 31, 2023. The datasets relevant to our research objectives were carefully selected and subsequently downloaded.

The data from Academic Torrents is stored in the .zst (Zstandard) file format, which necessitated decompression for further processing. To address this requirement, we employed scripts written in Swift, which efficiently converted the .zst files into the more accessible .json format. This conversion was a crucial step in our data preparation process, ensuring the data was in a usable form for subsequent analysis.

Following the decompression, the data was organized into a structured format to facilitate ease of access and analysis. Specifically, the decompressed .json files were split and reorganized into a month-year format. This systematic structuring was instrumental in enabling efficient data handling and retrieval, thereby streamlining the analytical processes that followed.

The implementation of these procedures was facilitated by custom scripts, the details of which are accessible via the link provided in the footnote \footnote{The code for the data collection process can be found at \url{https://git.uwaterloo.ca/jrwallace/PASS}.}. The time required for these processes varied significantly depending on the size of the datasets. Smaller datasets were processed in approximately 10 minutes, whereas larger datasets required up to 2 hours for complete decompression and reorganization.






\section{Dataset Description}
\subsection{Overview of Datasets}
We encompassed data from 12 subreddits covering six broad topics: gaming, technology, COVID-19, health, environment, and the University of Waterloo. Below is an overview of each dataset, highlighting the types of data, sources, and relevant characteristics. \footnote{Statistics updated upto May 25th 2024}

We consulted with the researchers to determine if they had specific dates or years in mind for analysis. If they did, we collected data for that specified duration. Otherwise, we utilized the entire dataset available. The reasons for selecting specific durations, when applicable, are detailed individually herein.

% \begin{enumerate}
%     \item \textbf{Gaming Subreddit}: The subreddit \textbf{r/disabledgamers} is a dedicated community where gamers with disabilities can seek assistance and share experiences related to gaming. Members of this subreddit discuss a variety of topics, including accessibility options, adaptive controls, and game mechanics tailored for individuals with disabilities. Additionally, the forum serves as a space for general discussions about gaming experiences, challenges, and successes, fostering a supportive and inclusive environment for all gamers. This subreddit has 9.1K members and amounts to be in the top 7\% by size. The data was collected from January 1, 2015, to December 31, 2023, and comprised 4,403 subreddit documents that were analyzed.


%     \item \textbf{Technology Subreddits}: These subreddits cover discussions on technological advancements. We analyzed 3 different technology based subreddits. 
%    \begin{enumerate}
%        \item  The subreddit \textbf{r/MachineLearning} is a vibrant community dedicated to discussions on machine learning, artificial intelligence, and data science. With over 2.9 million members, this subreddit serves as a hub for researchers, practitioners, and enthusiasts to share the latest research papers, industry news, project ideas, and technical questions. The community is highly active, regularly posting tutorials, code snippets, and hosting AMAs (Ask Me Anything) with prominent figures in the field. This subreddit is in the top 1\% by size, reflecting its significance and popularity among those interested in machine learning and AI. The researcher (Participant P2) was particularly interested in the latest innovations and discussions in the field of machine learning. Therefore, they chose to focus the analysis on the past year, specifically from January 1, 2023, to December 31, 2023, which comprised approximately 27,506 subreddit documents.

%        \item The subreddit \textbf{r/cybersecurity} is a comprehensive resource for anyone interested in the field of cybersecurity. With over 794K members, this subreddit covers a wide range of topics including threat analysis, security breaches, industry best practices, and career advice. Members frequently share news articles, research findings, and discussions about the latest security tools and techniques. This subreddit is in the top 1\% by size, indicating its crucial role as a go-to platform for cybersecurity professionals and enthusiasts. The researcher (Participant P4) aimed to explore the most recent trends and discussions in the field of cybersecurity. Consequently, they decided to limit the analysis to the past year, from January 1, 2023, to December 31, 2023, encompassing approximately 26,692 subreddit documents.

%        \item The subreddit \textbf{r/LanguageTechnology} focuses on the intersection of linguistics and technology, encompassing areas such as natural language processing (NLP), computational linguistics, and language-based AI. With over 48K members, this subreddit is a specialized community where researchers and practitioners discuss advancements, share research papers, and collaborate on projects related to language technologies. This subreddit is in the top 3\% by size, highlighting its importance for those engaged in the study and application of language technology. The data was collected from October 1, 2011 until December 31, 2023 amounting to contain 13,420 subreddit documents.
%    \end{enumerate}
   

%     \item \textbf{COVID-19 Subreddits and politics}: These include subreddits dedicated to discussions about the COVID-19 pandemic. Topics range from public health information and personal experiences, vaccines to policy discussions and politics, capturing the multifaceted nature of the pandemic. We analyzed 3 different COVID-19 based subreddits. 

% \begin{enumerate}
%     \item The subreddit \textbf{r/Coronavirus} is one of the largest and most comprehensive communities dedicated to discussions about the COVID-19 pandemic. With over 2.5 million members, this subreddit covers a wide range of topics including global news, scientific research, public health guidelines, and personal stories related to COVID-19. Members actively share the latest updates, ask questions, and provide support to one another during the ongoing pandemic. This subreddit is in the top 1\% by size, underscoring its critical role as a global information hub for COVID-19 related content. The researcher (Participant P10) was keen to examine the period when COVID-19 vaccines were first introduced. Therefore, the analysis was limited to the timeframe from November 1, 2020, to February 1, 2021, to investigate initial public reactions to COVID-19 and the vaccines. The focus was on understanding vaccine hesitancy and the political stance during that period, which encompassed approximately 23,906 subreddit documents.

%     \item The subreddit \textbf{r/CoronavirusCanada} focuses on discussions related to the COVID-19 pandemic within Canada. With over 16K members, this subreddit provides updates on local news, government policies, vaccination progress, and personal experiences related to COVID-19 in Canada. The community is a valuable resource for Canadians seeking information and support during the pandemic. This subreddit is in the top 5\% by size, reflecting its importance as a source of information and community support for Canadians. The researcher (Participant P12) aimed to understand the impact of COVID-19 in Canada from the onset of the pandemic. Therefore, the analysis was focused on the period from March 2020 until December 31, 2023, to capture the evolving discussions and topics throughout the years from start to end. This timeframe encompassed approximately 26,862 subreddit documents.

%     \item The subreddit \textbf{r/HermanCainAward} is a community where users document and discuss cases of individuals who publicly expressed skepticism about COVID-19 and subsequently experienced severe illness or death due to the virus. With over 492K members, this subreddit serves as a space for sharing stories, reflecting on the impact of misinformation, and promoting public health awareness. This subreddit is in the top 1\% by size, highlighting its significant engagement and controversial discussions surrounding the pandemic and vaccine skepticism. The researcher (Participant P3) sought to analyze the specific subreddit r/HermanCainAward from September 2021 until December 31, 2023, to understand people's interactions and responses within this community. This analysis period encompassed approximately 35,013 subreddit documents.
% \end{enumerate}

    

%     \item \textbf{Health Subreddits}: These subreddits focus on medical conditions, treatments, health advice, and wellness tips. The datasets are characterized by personal anecdotes and expert opinions, offering a comprehensive view of health-related discussions.

%  \begin{enumerate}
%      \item    The subreddit \textbf{r/emergencymedicine} is a specialized community dedicated to discussions about emergency medical care. With over 103K members, this subreddit serves as a hub for healthcare professionals, students, and enthusiasts to share experiences, seek advice, and discuss the latest advancements in emergency medicine. Topics include case studies, clinical guidelines, career advice, and personal stories from the field. This subreddit is in the top 10\% by size, reflecting its importance as a resource and support network for those involved in or interested in emergency medical care. The data was collected from April 1, 2012 until December 31, 2023, with 14,117 subreddit documents.

%  \item The subreddit \textbf{r/bipolar} is a supportive community for individuals affected by bipolar disorder, including those diagnosed with the condition, their families, and friends. With over 227K members, this subreddit offers a safe space for sharing personal experiences, coping strategies, and resources related to managing bipolar disorder. Discussions often include topics like medication, therapy, lifestyle changes, and mental health advocacy. This subreddit is in the top 5\% by size, underscoring its critical role as a support network for people dealing with bipolar disorder. The researcher (Participant P11) aimed to examine the most recent discussions related to bipolar disorder. Consequently, data was collected from June 1, 2023, to December 31, 2023, accounting for approximately 24,512 subreddit documents.

%  \item The subreddit \textbf{r/nutrition} is a vibrant community focused on all aspects of nutrition and dietary health. With over 4.5 million members, this subreddit provides a platform for sharing research, asking questions, and discussing various topics related to nutrition, including diet plans, nutritional science, supplements, and health outcomes. Members range from nutrition professionals and enthusiasts to individuals seeking advice on improving their diet. This subreddit is in the top 1\% by size, indicating its significant role in promoting nutritional education and healthy living. The researcher (Participant P8) aimed to explore the most recent food trends, diet plans, and discussions related to nutrition. Therefore, data was collected from January 1, 2023, to December 31, 2023, accounting for approximately 14,313 subreddit documents. 




     
%  \end{enumerate}
 

%     \item \textbf{Environment Subreddits}: This includes subreddits that discuss sustainability practices. The subreddit \textbf{r/sustainablefashion} is a dedicated community for individuals interested in eco-friendly and ethical fashion. With over 33K members, this subreddit serves as a platform for discussing sustainable fashion practices, sharing tips on how to create a more sustainable wardrobe, and exploring the environmental and social impacts of the fashion industry. Topics include upcycling, thrift shopping, sustainable brands, and DIY fashion projects. Members frequently share their experiences, advice, and knowledge on making fashion choices that are both stylish and environmentally responsible. This subreddit is in the top 3\% by size, highlighting its significance as a resource and community for those passionate about sustainability in fashion. Data collection was done from May 1, 2017 until December 31,2023 with 5845 subreddit documents to analyze.

  
%     \item \textbf{University of Waterloo Subreddit}: The subreddit \textbf{r/uwaterloo} is a vibrant community for students, alumni, faculty, and anyone interested in the University of Waterloo. With over 97K members, this subreddit serves as a central hub for discussions related to campus life, academic programs, student experiences, and university events. Topics frequently include course advice, co-op experiences, campus news, and social activities. Members share resources, ask questions, and provide support to one another, fostering a strong sense of community among those connected to the university. This subreddit is in the top 10\% by size, underscoring its importance as a resource and gathering place for the University of Waterloo community. The researcher (Participant P9) aimed to explore the recent events and discussions surrounding the University of Waterloo. Accordingly, data was gathered from January 1, 2023, to December 31, 2023, resulting in approximately 15,793 subreddit posts.
% \end{enumerate}

Table \ref{tab:dataset_descriptions} gives summary of the dataset description.  

% \begin{table}[h!]
%     \centering
%     \caption{Dataset Descriptions for Selected Subreddits POV 1}
%     \label{tab:dataset_descriptions}
%     \begin{tabular}{| p{4cm} | p{1cm} | p{2cm} | p{3cm} | p{3cm} |}
%         \hline
%         \textbf{Reddit} & \textbf{P ID } & \textbf{Modelling Documents} & \textbf{Start Date} & \textbf{End Date} \\ \hline
        
%         r/disabledgamers & P1 & 4403 & January 1, 2015 & December 31, 2023 \\ \hline
        
%         r/MachineLearning & P2 & 27506 & January 1, 2023 & December 31, 2023 \\ \hline
        
%     r/HermanCainAward & P3 & 35013 & September 1, 2021 & December 31, 2023 \\ \hline
    
%     r/cybersecurity & P4 & 26692 & January 1, 2023 & December 31, 2023 \\ \hline
    
%     r/emergencymedicine & P5 & 14117 & April 1, 2012 & December 31, 2023 \\ \hline
    
%     r/SustainableFashion & P6 & 5845 & May 1, 2017 & December 31, 2023 \\ \hline
    
%     r/LanguageTechnology & P7 & 13420 & October 1, 2011 & December 31, 2023 \\ \hline
    
%     r/nutrition & P8 & 14313 & January 1, 2023 & December 31, 2023 \\ \hline
    
%     r/uwaterloo & P9 & 15793 & January 1, 2023 & December 31, 2023 \\ \hline
    
%    r/Coronavirus & P10 & 23906 & November 1, 2020 & February 1, 2021 \\ \hline
   
%     r/bipolar & P11 & 24512 & June 1, 2023 & December 31, 2023 \\ \hline
    
%       r/CoronavirusCanada & P12 & 26862 & March 1, 2020 & December 31, 2023 \\ \hline
%     \end{tabular}
% \end{table}

\begin{table}[h!]
    \centering
    \caption{Dataset Descriptions for Selected Subreddits POV 2}
    \label{tab:dataset_descriptions}
    \begin{tabular}{ p{4cm}  p{1cm}  p{2.5cm}  p{3cm}  p{3cm} }
        \toprule
        \textbf{Subreddit} & \textbf{ID} & \textbf{Modelling Documents} & \textbf{Start Date} & \textbf{End Date} \\ 
        \midrule
        
        r/disabledgamers & P1 & 4,403 & 01/01/2015 & 31/12/2023 \\ 
        
        r/MachineLearning & P2 & 27,506 & 01/01/2023 & 31/12/2023 \\ 

        r/HermanCainAward & P3 & 35,013 & 01/09/2021 & 31/12/2023 \\ 

        r/cybersecurity & P4 & 26,692 & 01/01/2023 & 31/12/2023 \\ 
    
        r/emergencymedicine & P5 & 14,117 & 01/04/2012 & 31/12/2023 \\ 
    
        r/SustainableFashion & P6 & 5,845 & 01/05/2017 & 31/12/2023 \\ 
    
        r/LanguageTechnology & P7 & 13,420 & 01/10/2011 & 31/12/2023 \\ 
    
        r/nutrition & P8 & 14,313 & 01/01/2023 & 31/12/2023 \\ 
    
        r/uwaterloo & P9 & 15,793 & 01/01/2023 & 31/12/2023 \\ 
    
        r/Coronavirus & P10 & 23,906 & 01/11/2020 & 01/02/2021 \\ 
   
        r/bipolar & P11 & 24,512 & 01/06/2023 & 31/12/2023 \\ 
    
        r/CoronavirusCanada & P12 & 26,862 & 01/03/2020 & 31/12/2023 \\ 
        \bottomrule
    \end{tabular}
\end{table}



\section{Data Preprocessing}


The data loading begins by merging the submissions and comments from JSON files (\texttt{RS\_<filename>.json} and \texttt{RC\_<filename>.json}) located in a specific directory for the subreddit. If loading these files fails, the function logs an error message indicating the issue. This step is crucial as it retrieves the raw data that will be processed and analyzed in subsequent steps.

Once the data is loaded, the submissions and comments are merged into threads using their IDs. Submissions are identified by their ``id" field, while comments are linked to submissions by their ``link\_id" field. Each thread is constructed by combining its submission text (title and selftext) with the associated comments. This creates a cohesive narrative for each discussion thread. The merged threads are then saved into a JSON file for further processing, ensuring the data is organized and accessible for analysis.

The tokenization function begins by replacing specific characters in the documents to ensure consistency and readability. This includes converting Cyrillic characters to their Latin equivalents and removing unusual quotes and tags. After character replacement, the text is tokenized, which involves splitting the text into individual words or tokens. This is done using the \texttt{gensim} library's \texttt{simple\_preprocess} function, which also removes punctuation. The tokenized data is stored in a dictionary, mapping thread IDs to their respective token sets, preparing the data for the next stage of processing.

The first step in the cleaning process is removing stopwords, which are common words that do not contribute significant meaning to the text, such as ``and,'' ``the,'' and ``in.'' The function uses the NLTK library to identify and remove these words. Additionally, it filters out Reddit-specific terms and other irrelevant words to reduce noise in the dataset.

The function then identifies and retains frequently occurring word pairs, known as bigrams, using \texttt{gensim}'s \texttt{Phrases} model. This step is important because it helps in capturing common phrases that can provide more context than individual words. For example, the phrase ``machine learning'' would be treated as a single entity rather than two separate words.

Lemmatization is the process of converting words to their base or dictionary forms. The data cleaning function uses the \texttt{spaCy} library to perform lemmatization, focusing on nouns, adjectives, verbs, and adverbs. This step reduces the variability in the data by ensuring that different forms of a word (e.g., ``running,'' ``ran,'' and ``runs'') are treated as a single token (``run'').

To further improve interpretability, the function expands common acronyms and slang terms to their full forms. For instance, ``imo'' is converted to ``in my opinion'' and ``tbh'' is changed to ``to be honest.'' This ensures that all representations of these terms are standardized across the dataset.

The function performs a final cleanup by removing any remaining single characters and numeric tokens that do not contribute meaningful information. This ensures that only relevant tokens are retained for analysis. In the filtering step, we also remove the words ``removed'' and ``deleted'' to prevent them from interfering with the interpretation of other significant words.

After these steps, the cleaned and lemmatized token sets are ready for use in topic modeling or other analyses. The comprehensive cleaning process ensures that the data is of high quality, enhancing the accuracy and reliability of subsequent analytical results.




\section{Implementation}
The choice of LDA, NMF, and BERTopic for our study is driven by a combination of their individual strengths and the complementary insights they provide. LDA is chosen for its probabilistic approach and widespread acceptance in literature, making it a reliable and interpretable model. NMF offers computational efficiency and a matrix-based perspective that is fast and effective for large datasets. BERTopic leverages the cutting-edge capabilities of BERT to provide deep, contextually rich topic modeling.

\subsection{Hardware Specifications}
The experiments and model training were conducted on a MacBook Air equipped with the Apple M1 chip. This device featured an 8-core CPU, which includes 4 performance cores and 4 efficiency cores, providing a balanced blend of high performance and energy efficiency. Additionally, it is equipped with a 7-core GPU, designed to handle graphics-intensive tasks efficiently. The system is supported by 16GB of RAM memory, ensuring smooth and efficient processing of large datasets and complex computations. 




\subsection{Implementation of Latent Dirichlet Allocation (LDA) Model}


In this section, we describe the implementation of the Latent Dirichlet Allocation (LDA) model for topic modeling, focusing on the selection and justification of various parameters used in the process. The implementation was performed using the \texttt{gensim} library, with additional handling for multiprocessing and model evaluation metrics.

A dictionary is created from the token sets using \texttt{gensim}, compacted and saved. This dictionary maps each unique word to a unique ID. Subsequently, the token sets are converted to a bag-of-words corpus and serialized for later use. The corpus is then loaded for model training.

The model’s hyperparameters, \(\alpha\) and \(\eta\), are set on based default values:

\begin{itemize}
    \item \textbf{Alpha (\(\alpha\))}: Controls the distribution of topics per document. A \texttt{symmetric} value promotes a balanced topic distribution, while a lower value results in sparsity.
    \item \textbf{Eta (\(\eta\))}: Controls the distribution of words per topic. The \texttt{auto} setting allows the model to learn an asymmetric distribution.
\end{itemize}

These settings are critical as they influence the overall structure and interpretability of the generated topics.

The number of worker threads is determined based on the available CPU cores, with a minimum of one worker if the system has fewer than two cores. The LDA model is then trained using \texttt{gensim}'s \texttt{LdaMulticore}, which leverages multiple CPU cores to speed up the training process.

\begin{itemize}
    \item \textbf{Workers}: The number of CPU cores minus one is used to speed up the training process, 7 in this case.
    \item \textbf{Num Topics}: The optimal number of topics was chosen based on running the model with different values (5 to 50) and selecting the maximum topic coherence.

\end{itemize}


\subsection{Implementation of Non-Negative Matrix Factorization (NMF) Model}

In this section, we describe the implementation of the Non-Negative Matrix Factorization (NMF) model for topic modeling, focusing on the selection and justification of various parameters used in the process. The implementation was performed using the \texttt{scikit-learn} library, with additional handling for data transformation, model evaluation, and logging. The token sets are prepared by converting them into a text format suitable for the TF-IDF vectorizer. This involves joining the tokens into space-separated strings.
The TF-IDF vectorizer is then initialized and fitted to the token sets, transforming the text data into a TF-IDF matrix. This matrix is saved for future use. The NMF model is generated by fitting the TF-IDF matrix, ensuring reproducibility by setting a random state.

The number of topics (\texttt{num\_topics}) was chosen based on the maximum topic coherence value observed from running the model with different values ranging from 5 to 50 topics. This method ensures the optimal number of topics for the given dataset, balancing between detail and generality.


The NMF model training involves the following steps:

\begin{enumerate}
    \item \textbf{TF-IDF Vectorization}: The text data is transformed into a TF-IDF matrix using \texttt{TfidfVectorizer}. This step captures the importance of words in the context of the dataset by accounting for their frequency and distribution across documents.
    \item \textbf{Model Fitting}: The NMF model is fitted to the TF-IDF matrix. This process decomposes the TF-IDF matrix into two lower-dimensional matrices, identifying the latent topics within the text data.
\end{enumerate}

\subsection{Implementation of BERTopic Model}

In this section, we describe the implementation of the BERTopic model for topic modeling, focusing on the selection and justification of various parameters used in the process. The implementation leverages advanced techniques in natural language processing (NLP) and machine learning, including the Sentence-BERT model, UMAP for dimensionality reduction, HDBSCAN for clustering, and cTF-IDF for topic extraction. The token sets are prepared by converting them into a text format suitable for the BERTopic model. This involves joining the tokens into space-separated strings.

The BERTopic model is then initialized with several components:

\begin{itemize}
    \item \textbf{Embedding Model}: The Sentence-BERT model (\texttt{all-MiniLM-L6-v2}), which is the default model, is used to generate dense vector representations (embeddings) of the texts. Sentence-BERT is chosen for its ability to produce high-quality embeddings that capture semantic meaning.
    \item \textbf{Dimensionality Reduction}: UMAP (Uniform Manifold Approximation and Projection) is used to reduce the dimensionality of the embeddings. UMAP is configured with 15 neighbors, 5 components, a minimum distance of 0.0, and a cosine metric, which helps in maintaining the local and global structure of the data.
    \item \textbf{Clustering}: HDBSCAN (Hierarchical Density-Based Spatial Clustering of Applications with Noise) is used for clustering the reduced embeddings. HDBSCAN is chosen for its robustness in identifying clusters of varying shapes and densities. It is configured with a minimum cluster size of 15, an euclidean metric, and the EOM (Excess of Mass) method for cluster selection.
    \item \textbf{Vectorization}: CountVectorizer is used to tokenize the topics, with English stop words removed to improve the quality of the topics.
    \item \textbf{Class-Based TF-IDF}: The ClassTfidfTransformer is used to extract the topic words based on the TF-IDF scores of the terms within each class (topic).
\end{itemize}


Furthermore, \cite{allaoui2020considerably} showed that utilizing UMAP for reducing high-dimensional embeddings can enhance the performance of established clustering algorithms like k-Means and HDBSCAN, improving both clustering accuracy and processing time.

The BERTopic model is then configured to calculate topic probabilities and is set to automatically determine the optimal number of topics. In the BERTopic model, the \texttt{nr\_topics} parameter controls the number of topics that the model will generate. Setting \texttt{nr\_topics} to \texttt{"auto"} allows the model to automatically determine the optimal number of topics based on the data. This automatic determination helps in diversifying the topic words and ensures that the number of topics is neither too large nor too small, thereby improving the coherence and interpretability of the topics. The model dynamically merges similar topics to provide a more concise and meaningful set of topics, enhancing the overall quality of the topic modeling output.

To determine an optimal value for \texttt{nr\_topics}, we ran the model 11 times and then chose the median value. Since BERTopic can yield different numbers of topics in each run due to its stochastic nature, this approach provides statistical significance by reducing the impact of outliers and ensuring a robust selection of the number of topics. Additionally, we observed that the mean and median values for \texttt{nr\_topics} were almost in conjunction, differing by an average standard deviation of \(\pm 1.349\) across 12 datasets. This small deviation further validates the stability and reliability of the chosen \texttt{nr\_topics} value.




===================

%======================================================================
\chapter{Pilot Study }
%======================================================================




   %\section{Introduction}
       
        %     The objective of this pilot study was to conduct preliminary investigations before commencing the actual interviews. The primary aim was to gather feedback on the study design, conceptual understanding, and operational procedures. Additionally, the pilot study served as an opportunity to run a demonstration of the research process and identify potential challenges that may arise during actual data collection.

        %     One of the main motivations for conducting the pilot study was to obtain early feedback from HCI researchers. By involving individuals with diverse expertise, we aimed to gather valuable insights and perspectives that could inform improvements to the research methodology.  
       
     
        % The research design involved a structured approach to gather feedback and insights from participants within the Human-Computer Interaction (HCI) group. The study setting, situated in the Games Institute (GI) meeting room, provided a conducive environment for the presentation and discussion of research findings. Through a concise 10-minute presentation, supplemented by interactive engagement, participants were invited to inquire and provide feedback. This interactive approach encouraged active participation, enabling participants to not only inquire but also contribute their perspectives, discussing and promoting a collaborative exchange of ideas.

We conducted a pilot study to carry out preliminary investigations before starting the actual interviews. Our primary aim was to gather feedback on the study design, conceptual understanding, and operational procedures. Additionally, we used the pilot study to demonstrate the research process and identify potential challenges for actual data collection.

By involving researchers from the Human-Computer Interaction (HCI) group, with diverse expertise, we aimed to gather valuable insights and perspectives to improve the research methodology. The Games Institute (GI) meeting room provided a conducive environment for presenting and discussing our findings. We delivered a concise 10-minute presentation, encouraging participants to ask questions and provide feedback. This interactive approach promoted active participation and a collaborative exchange of ideas.
     
        
   \section{Participants}

    
       Ten HCI researchers participated in the study, including four professors, one postdoctoral researcher, and five master's students. They brought expertise in thematic analysis, user experience (UX) research, and immersive technologies like gaming and virtual reality. All participants were fluent in English.

       
    \section{Data Collection and Analysis}
    
       We chose the \textit{r/uwaterloo} subreddit as our primary data source because of its lively and engaged community, which is relevant to the study's themes and the participants involved. Data collection was facilitated through web scraping techniques implemented using custom scripts discussed in \autoref{data_collect}. The chosen timeframe for analysis was January 1st to December 31st, 2023 (01/01/2023 - 31/12/2023). The collected data, comprising comments and submissions, amounted to 10,413 documents, ensuring a comprehensive representation of community interactions and discussions.

       
        With this extensive dataset, the subsequent phase involved the application of three distinct topic modeling algorithms: Latent Dirichlet Allocation (LDA), Top2Vec, and BERTopic. 
        LDA uses probabilistic distributions for interpretability, Top2Vec embeds topics and documents in the same vector space for semantic relationships, and BERTopic leverages BERT embeddings and HDBSCAN for high coherence and precise clustering.
        The resulting outputs, consisting of topic keywords generated by each algorithm, were meticulously documented and subsequently transcribed into hardcopy format for qualitative and analytical interpretation.

       
    
    We began the data collection process with each participant analyzing the outcomes derived from the three distinct topic modeling algorithms: Latent Dirichlet Allocation (LDA), Top2Vec, and BERTopic. Following this analysis, participants provided their insights and responded to a series of questions outlined in the second phase of the interview protocol. These questions were meticulously designed to delve into the participants' perceptions, interpretations, and preferences regarding the generated results.
    
    
        The data analysis phase involved two distinct components: a quantitative analysis that focused on the statistical results and a qualitative examination that involved gathering subjective feedback from the participants. Although the primary focus of the pilot study was on qualitative insights, the statistical findings provided supplementary information that aligned with our overarching objectives.

    
        In parallel, the qualitative analysis involved a meticulous examination of the participants' responses, aiming to extract nuanced insights and perspectives. Each participant's feedback was carefully reviewed, and a comprehensive summary document was compiled to highlight the key points and observations shared by the participants. 



        \section{Procedure}
As part of the research protocol, we provided each participant with a hard copy of the Microsoft Desirability Toolkit \cite{benedek2010measuring, rohrer2008desirability}. This toolkit, a renowned resource, helps elicit subjective assessments and insights about user experience. It proved to be valuable during the interview phase, where participants expressed their insights for each model's results and chose the adjectives that best suited the results according to their understanding.  Additionally, participants were presented with a set of interview questions (Interview Questions Phase II, \autoref{tab:interview_phase2}) to gather insights after interacting with the results produced by the three models.

We also provided participants with hard copies of the detailed results generated by each topic modeling algorithm, including Latent Dirichlet Allocation (LDA), Top2Vec, and BERTopic. These supplementary materials offered comprehensive insights into the thematic structures identified within the dataset by these models. You can find the detailed results in the Appendix.
        
After participants completed the analysis and responded to the interview questions, the session transitioned into an open discussion format. During this interactive segment, participants were encouraged to share their insights, provide feedback, articulate their comments, and elucidate their rationale behind selecting a specific model. Additionally, participants engaged in discussions surrounding the criteria for ranking the models, considering factors such as their comprehension, familiarity, and acceptance of the results. This collaborative exchange fostered a rich and insightful dialogue, enhancing the overall depth and breadth of the research findings.


        
  \section{Results}
     \subsection{Quantitative Results }
     
         The quantitative analysis revealed that BERTopic achieved the highest performance in terms of topic coherence, followed by LDA, with Top2Vec demonstrating the lowest topic coherence. Regarding topic diversity, both BERTopic and LDA outperformed Top2Vec, with BERTopic leading in this metric. In terms of runtime and execution, LDA was the fastest, followed by Top2Vec, with BERTopic taking the longest time. These findings are summarized and presented in \autoref{tab:model_performance}.



\begin{table}[h!]
    \centering
    \scriptsize
    \caption{Summary of Model Performance: Pilot study}
    \label{tab:model_performance}
    \begin{tabular}{ p{3cm} p{3cm} p{3cm} p{3cm} }
        \toprule
        \textbf{Model} & \textbf{Topic Coherence} & \textbf{Topic Diversity} & \textbf{Run Time (seconds)} \\ 
        \midrule
        BERTopic & 0.62 & 1 & 270 \\ 
        LDA & 0.56 & 1 & 25 \\
        Top2Vec & 0.36 & 0.67 & 258 \\ 
        \bottomrule
    \end{tabular}
   
\end{table}




 

    \subsection{Qualitative Results }



        In the pilot study conducted with 10 participants, the evaluation of different topic modeling algorithms revealed varied insights into their usability, interpretability, and overall effectiveness. Among the three models assessed --- BERTopic, Top2Vec, and LDA --- participants exhibited varying preferences and provided diverse feedback, shedding light on the strengths and limitations of each approach. \autoref{tab:model_comparison} discusses the words selected by participants from the Microsoft Disability Toolkit for answering question 1 of interview phase II.

        Participants' feedback highlighted key differences among the three topic modeling algorithms. BERTopic emerged as the most favored choice, with five participants ranking it highest. They praised its comprehensive results, intuitive presentation, and logical grouping of topics, making it easy to navigate and interpret. The inclusion of confidence intervals (probabilities) provided additional context, boosting confidence in the model's output. However, some found BERTopic's results complex and overwhelming, particularly the probability numbers. Overall, the consensus was that BERTopic's topics were meaningful and coherent, contributing to a satisfying user experience.

Top2Vec received mixed feedback, with three participants ranking it as their top choice. While some appreciated its representational capabilities and semantic coherence, others found it challenging to navigate due to the abundance of words and lack of numerical values. Participants noted that Top2Vec's keywords were clear but felt less reliable without accompanying numbers. Despite these challenges, some found Top2Vec to be simple, useful, and fitting their impressions of UWaterloo. LDA, on the other hand, garnered the least enthusiasm. Participants found its topics irrelevant and its statistical aspects confusing and frustrating. Nonetheless, a few appreciated the qualitative and quantitative comparison it offered. Notably, one participant switched their preference from LDA to BERTopic after discussions, underscoring the impact of collaborative deliberation. Overall, the study underscored the importance of user perspectives in evaluating topic modeling algorithms and guided future protocols for the main user studies.



        % \subsubsection{BERTopic}
        
        % BERTopic emerged as the most favored choice among participants, with 5 participants ranking it as their top choice. Participants commended BERTopic for its comprehensive results and intuitive presentation. The logical grouping of topics resonated well with users, who found it easy to navigate and interpret. 
        
        % For instance, participant P1 stated, \textit{``Bertopic cleanly groups and orders relevant words by `topic'/ `context'. I can see this being easy to understand and use".} 
        
        % The inclusion of confidence intervals (probabilities) provided additional context, boosting participants' confidence in the model's output.
        
        % Participants P5 stated, \textit{``I like being able to see the values associated with words in Bertopic"}, while participant P7 stated that they also liked the confidence values in Bertopic. Participant P3 also mentioned that, \textit{``Bertopic had more `pleasant' words from the Microsoft Desirability toolkit as compared to the LDA model [as their answer to Q1]." }
        
        % Some participants found the model results complex to interpret and overwhelming. For example, participant P8 stated that, \textit{``Bertopic numbers looks too complex, difficult to compare. The words are easy to understand but probability numbers are complex"}. 
        
        % Nevertheless, the general consensus was that BERTopic's topics were meaningful and coherent, contributing to a `satisfying’ user experience overall. 

        % \subsubsection{Top2Vec}
        
        % Conversely, Top2Vec gathered mixed feedback from participants, with 3 participants ranking it as their top choice.  While some appreciated its representational capabilities and semantic coherence, others found it challenging to navigate due to the abundance of words and the lack of numerical values.

        % For instance, participant P5 stated that, \textit{``The keywords for top2vec are very clear but not having any numbers along side it make it feel less reliable" }. Participants P9 and P10 found the Top2Vec presentation to be the best, but it lacked the information about counts/frequency for context. In accordance with them, participant P8 states, \textit{``[Top2Vec] probably the most easy for humans to understand, simple and useful"}

        % Participant P6 found Top2Vec ``fits their own impression of UWaterloo". They stated, \textit{I like how Top2Vec is creating keywords based on some sort of `stereotype' of mine. Overall Top2Vec is more academic than the other two [models] which is my deepest impression of the topic".}
        
        
        % The overlapping nature of topics further compounded the difficulty in interpreting results. Despite these challenges, one participant found Top2Vec's results `entertaining’, suggesting potential engagement benefits despite its complexities.


        % \subsubsection{LDA}
        
        % In contrast, participants expressed less enthusiasm for LDA. Many found its topics to be irrelevant and lacking in predictive accuracy. For instance, participant P7 stated, \textit{``I had a hard time figuring out why/ how the keywords are connected the topics did not make sense to me".}
        
        % Some participants reported confusion and frustration with the results, especially the statistical aspects associated with LDA. Participant P1 stated that, \textit{`` [I am] unsure what numeric stats mean, words in group [are] not relevant?"}. On similar grounds, participant P5 found \textit{`` for LDA the values are not useful because you don't know what to focus on."} However, participant P8 liked \textit{``the qual[itative] + quant[itaive] side by side; help to filter saliency of themes."}
        
        % Notably, one participant switched their preference from LDA to BERTopic after engaging in discussions, highlighting the impact of collaborative deliberation on decision-making processes.
        
        % Overall, the pilot study underscored the importance of considering user perspectives and preferences when evaluating topic modeling algorithms. While BERTopic emerged as the preferred choice for its comprehensive and intuitive results, Top2Vec and LDA also offered unique insights and functionalities. The diverse feedback provided by participants illuminated the strengths and limitations of each model, guiding future protocols to be incorporated in the main user studies. 





      
 \begin{table}
  
    \centering
    \scriptsize
     \caption{Comparison of Attributes Across Models: Microsoft Desirability Toolkit}
    \label{tab:model_comparison}
     \begin{tabular}{ p{3cm} p{3cm} p{3cm} p{3cm} }
      \toprule
        \textbf{BERTopic} & \textbf{Top2Vec} & \textbf{LDA} \\
       \midrule
        Accessible & Understandable & Understandable \\
        Clean & Accessible & Clean \\
        Organized & Relevant & Incomprehensible \\
        Reliable & Organized & Inconsistent \\
        Consistent & Familiar & Undesirable \\
        Understandable & Expected & Ineffective \\
        Meaningful & Simplistic & Overwhelming \\
        Satisfying & Entertaining & Irrelevant \\
        Relevant & Usable & Not Valuable \\
        Expected & Inconsistent & Poor quality \\
        Useful & Intuitive & Incomprehensible \\
        Predictable & Hard to Use & Confusing \\
        Convenient & Inconsistent & Difficult \\
        Overwhelming & Intimidating & Unrefined \\
        Rigid & Overwhelming & Hard to Use \\
        Disconnected & Busy & Unattractive \\
        & Time-consuming  & \\
        & Unattractive & \\
        &  Unrefined & \\
          \bottomrule
    \end{tabular}
     
\end{table}
    
    \section{Discussion}

    
        Based on the insights gathered from the pilot study, it is evident that each model, BERTopic, Top2Vec, and LDA, offers unique advantages and limitations. BERTopic emerged as the preferred choice among participants, commended for its comprehensive and easily interpretable results. Participants appreciated its semantic grouping of topics, clear ranking presentation, and the confidence interval feature, which enhanced decision-making. Conversely, Top2Vec was praised for its representability and ability to capture the essence of the subreddit's content. However, concerns were raised about the abundance of words, lack of numerical values, and overlapping topics. LDA, while offering statistical insights, fell short in relevance and predictive accuracy, leading to participant confusion and dissatisfaction. Interestingly, after group discussion, a participant revised their ranking, favoring BERTopic over LDA, underscoring the importance of collaborative evaluation in refining perceptions. 

        Furthermore, these results align with our statistical analysis, which demonstrated that BERTopic outperformed both LDA and Top2Vec in terms of topic coherence and semantic grouping. Specifically, BERTopic exhibited superior performance, followed by LDA, while Top2Vec showed the least coherence. In terms of topic diversity, BERTopic and LDA surpassed Top2Vec. 


        
After conducting the pilot study, we recognized the need for methodological adjustments. The study highlighted the superior performance of BERTopic in terms of topic coherence, semantic grouping, and diversity. Given its similarities to Top2Vec, we opted to replace Top2Vec with Non-Negative Matrix Factorization (NMF) for greater efficiency. NMF was chosen for its faster performance and its matrix-based approach, which differs from the probabilistic methods of LDA and neural-network methods of BERTopic.

The choice of LDA, NMF, and BERTopic for our study is driven by a combination of their individual strengths and the complementary insights they provide. LDA is chosen for its probabilistic approach and widespread acceptance in literature, making it a reliable and interpretable model. NMF offers computational efficiency and a matrix-based perspective that is fast and effective for large datasets. BERTopic leverages the cutting-edge capabilities of BERT to provide deep, contextually rich topic modeling.

Participant feedback emphasized the necessity for consistent visualization, leading to the incorporation of BERTopic into the Computational Thematic Analysis toolkit. Additionally, discussions with participants revealed that they were more articulate when speaking rather than writing. Consequently, we structured our user studies as semi-structured interviews, allowing us to transcribe their responses for analysis. 
    
        
   \section{Conclusion}
     
     This pilot study provided valuable insights into the performance and suitability of three topic modeling techniques—BERTopic, LDA, and Top2Vec—for analyzing textual data from the r/uwaterloo subreddit. Through a comprehensive analysis of participant feedback and statistical results, BERTopic emerged as the most effective method, demonstrating superior performance in terms of topic coherence, semantic grouping, and diversity. The results also highlighted the importance of considering both quantitative and qualitative factors when evaluating the efficacy of topic modeling algorithms. Furthermore, the collaborative discussion among participants facilitated a deeper understanding of the strengths and limitations of each model, leading to informed decision-making and potential revisions in model preferences. 
     
      Moving forward, the insights gained from this study will inform the selection and implementation of topic modeling techniques for the main user case study.

      
        


% \section{Visualizations}







% - using watgpu,bertopioc processig time can be increased, \\
% can prep priocessing in bertipic be a factor ?? \\
% Coz lda, nmf take mich more iterative approach for data cleaning, what if bertopic missied some imp parts\\


% \textbf{Perplexity}
% BERTopic's consistently low perplexity scores indicate its strength in accurately modeling the underlying data, which is beneficial for analyses requiring precise data representation. The integration of BERT embeddings in BERTopic helps capture semantic relationships between words, improving model perplexity \cite{grootendorst2022bertopic}. Low perplexity is associated with better generalization and predictive performance in topic models \cite{lau2014machine}. NMF, while not as effective as BERTopic, still shows reasonable performance and is useful for applications preferring simpler models \cite{lee2001algorithms}. NMF's parts-based representation allows for clear and interpretable topic clusters despite its higher perplexity scores. LDA, with higher perplexity scores, may be less effective in capturing data complexity but offers a probabilistic approach useful in specific contexts \cite{griffiths2007probabilistic}. LDA balances broad themes and detailed subtopics, suitable for applications requiring a trade-off between accuracy and interpretability.

% The utility of low perplexity in enhancing topic model performance is underscored by its indication of a better fit to the data and improved model applicability \cite{blei2003latent}. Thus, BERTopic's consistent low perplexity scores highlight its potential utility in various applied contexts, ensuring reliable and high-quality outcomes.












==> figures.tex <==
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P1/lda.png}
\fbox{\includegraphics[width=1\textwidth]{P1/lda_topics.png}}
 
  
    
    \caption{LDA Topic keywords for LDA for Dataset: r/disabledgamers}
    \label{fig:lda_nmf}
\end{figure}


% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P1/nmf.png}
      \fbox{\includegraphics[width=1\textwidth]{P1/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/disabledgamers}

    \label{fig:2}
\end{figure}


% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P1/bertopic.png}
     \fbox{  \includegraphics[width=1\textwidth]{P1/bertopic_topics.png}}
   \caption{Topic keywords for BERTopic for Dataset: r/disabledgamers}
    \label{fig:3}
\end{figure}



\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P2/lda.png}
    \fbox{ \includegraphics[width=1\textwidth]{P2/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/machinelearning}
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P2/nmf.png}
   \fbox{ \includegraphics[width=1\textwidth]{P2/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/machinelearning}
    \label{fig:5}

\end{figure}


% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P2/bertopic.png}
  
    \caption{Topic keywords for BERTopic for Dataset: r/machinelearning}
    \label{fig:6}

\end{figure}




% Third image on the next page
\begin{figure}[tb!]
    \centering
     \fbox{\includegraphics[width=1\textwidth]{P2/bertopic_topics.png}}
\fbox{\includegraphics[width=1\textwidth]{P2/bertopic_small.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/machinelearning (continued)}
    \label{fig:6}

\end{figure}







\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P3/lda.png}
\fbox{\includegraphics[width=0.9\textwidth]{P3/lda_topics.png}}
    \caption{ Topic keywords for LDA for Dataset: r/HermanCainAward}
    \label{fig:lda_nmf}
\end{figure}






\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P3/nmf.png}
  \fbox{\includegraphics[width=0.9\textwidth]{P3/nmf_topics.png}}
    \caption{ Topic keywords for NMF for Dataset: r/HermanCainAward}
    \label{fig:lda_nmf}
\end{figure}

   
% \begin{figure}[tb!]
%     \centering
    
%     \caption{ Topic keywords for NMF for Dataset: r/HermanCainAward}
%     \label{fig:lda_nmf}
% \end{figure}


\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P3/bertopic_hca.png}
\fbox{\includegraphics[width=1\textwidth]{P3/bertopic_1.png}}
    \caption{ Topic keywords for BERTopic for Dataset: r/HermanCainAward}
    \label{fig:lda_nmf}
\end{figure}

   


\begin{figure}[tb!]
    \centering
      \fbox{\includegraphics[width=1\textwidth]{P3/bertopic_2.png}}
       \fbox{\includegraphics[width=1\textwidth]{P3/bertopic_3.png}}
    \caption{ Topic keywords for BERTopic for Dataset: r/HermanCainAward (continued)}
    \label{fig:lda_nmf}
\end{figure}


% \begin{figure}[tb!]
%     \centering
     
%     \caption{ Topic keywords for BERTopic for Dataset: r/HermanCainAward}
%     \label{fig:lda_nmf}
% \end{figure}








\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P4/lda_cyber_final.png}
    \fbox{ \includegraphics[width=1\textwidth]{P4/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/cybersecurity}
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P4/nmf_cyber.png}
   \fbox{ \includegraphics[width=1\textwidth]{P4/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/cybersecurity}
    \label{fig:5}

\end{figure}


% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P4/bertopic_cyber.png}
    \fbox{\includegraphics[width=1\textwidth]{P4/b1.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/cybersecurity}
    \label{fig:6}

\end{figure}






% Third image on the next page
\begin{figure}[tb!]
    \centering
\fbox{\includegraphics[width=0.9\textwidth]{P4/b2.png}}
\fbox{\includegraphics[width=0.9\textwidth]{P4/b3.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/cybersecurity (continued)}
    \label{fig:6}

\end{figure}

% % Third image on the next page
% \begin{figure}[tb!]
%     \centering

%     \caption{Topic keywords for BERTopic for Dataset: r/cybersecurity (contd)}
%     \label{fig:6}

% \end{figure}









\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P5/LDA_em.png}
    \fbox{ \includegraphics[width=1\textwidth]{P5/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/emergencymedicine}
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P5/NMF_EM.png}
   \fbox{ \includegraphics[width=0.8\textwidth]{P5/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/emergencymedicine}
    \label{fig:5}

\end{figure}


% % Third image on the next page
% \begin{figure}[tb!]
%     \centering

%     \caption{Topic keywords for NMF for Dataset: r/emergencymedicine}
%     \label{fig:6}

% \end{figure}


% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P5/bertopic_EM.png}
    \fbox{\includegraphics[width=1\textwidth]{P5/bertopic_topics.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/emergencymedicine}
    \label{fig:6}

\end{figure}








\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P6/lda_Sfashion.png}
    \fbox{ \includegraphics[width=1\textwidth]{P6/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/SustainableFashion}
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P6/NMF_Sfashion.png}
   \fbox{ \includegraphics[width=1\textwidth]{P6/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/SustainableFashion}
    \label{fig:5}

\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P6/bertopic_Sfashion.png}
    \fbox{\includegraphics[width=0.8\textwidth]{P6/bertopic_topics.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/SustainableFashion}
    \label{fig:6}

\end{figure}


% Third image on the next page
% \begin{figure}[tb!]
%     \centering
    
    
%     \caption{Topic keywords for BERTopic for Dataset: r/SustainableFashion}
%     \label{fig:6}

% \end{figure}







\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P7/lda_ltech.png}
    \fbox{ \includegraphics[width=1\textwidth]{P7/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/LanguageTechnology }
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P7/nmf_ltech.png}
   \fbox{ \includegraphics[width=1\textwidth]{P7/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/LanguageTechnology }
    \label{fig:5}

\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P7/bertopic_ltech.png}
     \fbox{\includegraphics[width=0.8\textwidth]{P7/b1.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/LanguageTechnology }
    \label{fig:6}

\end{figure}


% % Third image on the next page
% \begin{figure}[tb!]
%     \centering
    
   
%     \caption{Topic keywords for BERTopic for Dataset: r/LanguageTechnology }
%     \label{fig:6}

% \end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    
    \fbox{\includegraphics[width=1\textwidth]{P7/b2.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/LanguageTechnology (continued) }
    \label{fig:6}

\end{figure}







\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P8/LDa.png}
    \fbox{ \includegraphics[width=1\textwidth]{P8/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/nutrition }
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P8/NMf.png}
   \fbox{ \includegraphics[width=1\textwidth]{P8/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/nutrition }
    \label{fig:5}

\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P8/bertopic_nutrition.png}
       \fbox{\includegraphics[width=1\textwidth]{P8/bertopic_topics.png}}
    
    \caption{Topic keywords for BERTopic for Dataset: r/nutrition }
    \label{fig:6}

\end{figure}








\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P9/LDA.png}
    \fbox{ \includegraphics[width=1\textwidth]{P9/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/Coronavirus }
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P9/nmf.png}
   \fbox{ \includegraphics[width=1\textwidth]{P9/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/Coronavirus }
    \label{fig:5}

\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P9/bertopic.png}
    \fbox{ \includegraphics[width=1\textwidth]{P9/b1.png}}
    
    \caption{Topic keywords for BERTopic for Dataset: r/Coronavirus }
    \label{fig:6}

\end{figure}




% Third image on the next page
\begin{figure}[tb!]
    \centering
   \fbox{ \includegraphics[width=1\textwidth]{P9/b2.png}}
     \fbox{ \includegraphics[width=1\textwidth]{P9/b3.png}}
    
    \caption{Topic keywords for BERTopic for Dataset: r/Coronavirus (continued)}
    \label{fig:6}

\end{figure}


% % Third image on the next page
% \begin{figure}[tb!]
%     \centering
  
    
    
%     \caption{Topic keywords for BERTopic for Dataset: r/Coronavirus }
%     \label{fig:6}

% \end{figure}






\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P10/LDA.png}
    \fbox{ \includegraphics[width=1\textwidth]{P10/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/uwaterloo }
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P10/nmf.png}
   \fbox{ \includegraphics[width=1\textwidth]{P10/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/uwaterloo }
    \label{fig:5}

\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P10/bertopic.png}
      
     \fbox{ \includegraphics[width=0.8\textwidth]{P10/bertopic_topics.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/uwaterloo }
    \label{fig:6}

\end{figure}


\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P11/LDA.png}
    \fbox{ \includegraphics[width=1\textwidth]{P11/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/bipolar}
    \label{fig:4}
  
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P11/NMF.png}
   \fbox{ \includegraphics[width=1\textwidth]{P11/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/bipolar}
    \label{fig:5}
\end{figure}



% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P11/bertopic.png}
    \fbox{\includegraphics[width=1\textwidth]{P11/b1.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/bipolar}
    \label{fig:6}
\end{figure}


% Third image on the next page
\begin{figure}[tb!]
    \centering
\fbox{\includegraphics[width=1\textwidth]{P11/b2.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/bipolar (continued)}
    \label{fig:6}
\end{figure}



\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P12/lda.png}
    \fbox{ \includegraphics[width=1\textwidth]{P12/lda_topics.png}}
    \caption{Topic keywords for LDA for Dataset: r/CoronavirusCanada}
    \label{fig:4}
\end{figure}

% Third image on the next page
\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P11/NMF.png}
   \fbox{ \includegraphics[width=1\textwidth]{P12/nmf_topics.png}}
    \caption{Topic keywords for NMF for Dataset: r/CoronavirusCanada}
    \label{fig:5}
\end{figure}


\begin{figure}[tb!]
    \centering
    \includegraphics[width=1\textwidth]{P12/bertopic.png}
   \fbox{ \includegraphics[width=1\textwidth]{P12/b1.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/CoronavirusCanada}
    \label{fig:5}
\end{figure}



\begin{figure}[tb!]
    \centering
   
   \fbox{ \includegraphics[width=1\textwidth]{P12/b2.png}}
    \caption{Topic keywords for BERTopic for Dataset: r/CoronavirusCanada (continued)}
    \label{fig:5}
\end{figure}





==> glossaries.tex <==
% Main glossary entries -- definitions of relevant terminology
\newglossaryentry{computer}
{
name=computer,
description={A programmable machine that receives input data,
               stores and manipulates the data, and provides
               formatted output}
}

% Nomenclature glossary entries -- New definitions, or unusual terminology
\newglossary*{nomenclature}{Nomenclature}
\newglossaryentry{dingledorf}
{
type=nomenclature,
name=dingledorf,
description={A person of supposed average intelligence who makes incredibly brainless misjudgments}
}

% List of Abbreviations (abbreviations type is built in to the glossaries-extra package)
\newabbreviation{aaaaz}{AAAAZ}{American Association of Amateur Astronomers and Zoologists}

% List of Symbols
\newglossary*{symbols}{List of Symbols}
\newglossaryentry{rvec}
{
name={$\mathbf{v}$},
sort={label},
type=symbols,
description={Random vector: a location in n-dimensional Cartesian space, where each dimensional component is determined by a random process}
}

==> math.tex <==
% \chapter {Mathematics}
% \section{Explanation of SBERT, UMAP, HDBSCAN, and c-TF-IDF with Mathematical Formulations}

% This section provides a detailed breakdown of the key components used in BERTopic: SBERT, UMAP, HDBSCAN, and c-TF-IDF. Each of these components plays a crucial role in generating meaningful and contextually relevant topics from text data.

% \subsection{SBERT: Sentence-BERT}

% Sentence-BERT (SBERT) is an adaptation of the BERT model designed for producing semantically meaningful sentence embeddings. It is particularly useful for tasks such as semantic textual similarity, clustering, and information retrieval. SBERT modifies the original BERT architecture to handle sentence-level tasks more efficiently.

% \subsubsection{Input Representation}

% SBERT takes as input a pair of sentences \( (s_1, s_2) \). Each sentence is tokenized into a sequence of word pieces using the WordPiece tokenizer. The tokenized sequences are:

% \[
% \mathbf{S_1} = [CLS, t_1^1, t_2^1, \ldots, t_n^1, SEP]
% \]

% \[
% \mathbf{S_2} = [CLS, t_1^2, t_2^2, \ldots, t_m^2, SEP]
% \]

% where \( [CLS] \) is the classification token and \( [SEP] \) is the separator token. \( t_i^1 \) and \( t_j^2 \) represent the tokens in sentences \( s_1 \) and \( s_2 \), respectively.

% \subsubsection{BERT Encoding}

% The tokenized sequences are passed through the BERT model to obtain contextualized embeddings for each token. Let \( \mathbf{H}_i \) represent the hidden states of the tokens in the \( i \)-th layer of BERT. For the final layer, we have:

% \[
% \mathbf{H}_{\mathbf{S_1}} = BERT(\mathbf{S_1})
% \]

% \[
% \mathbf{H}_{\mathbf{S_2}} = BERT(\mathbf{S_2})
% \]

% \subsubsection{Sentence Embedding}

% To obtain a fixed-size sentence embedding, SBERT typically uses the embedding of the [CLS] token from the final layer, which is designed to capture the aggregate representation of the sentence. The sentence embeddings \( \mathbf{E}(s_1) \) and \( \mathbf{E}(s_2) \) are given by:

% \[
% \mathbf{E}(s_1) = \mathbf{H}_{\mathbf{S_1}}^{[CLS]}
% \]

% \[
% \mathbf{E}(s_2) = \mathbf{H}_{\mathbf{S_2}}^{[CLS]}
% \]

% Alternatively, SBERT can use mean pooling over all token embeddings to derive the sentence embeddings:

% \[
% \mathbf{E}(s) = \frac{1}{n} \sum_{i=1}^{n} \mathbf{H}_i
% \]

% where \( n \) is the number of tokens in the sentence.

% \subsubsection{Training Objective}

% SBERT is typically trained using a Siamese or triplet network structure with a distance-based loss function, such as cosine similarity or Euclidean distance. For semantic textual similarity tasks, the cosine similarity between two sentence embeddings is calculated as:

% \[
% \text{sim}(\mathbf{E}(s_1), \mathbf{E}(s_2)) = \frac{\mathbf{E}(s_1) \cdot \mathbf{E}(s_2)}{\|\mathbf{E}(s_1)\| \|\mathbf{E}(s_2)\|}
% \]

% The training objective is to minimize the difference between the predicted similarity scores and the ground truth similarity scores.

% \subsection{UMAP: Uniform Manifold Approximation and Projection}

% Uniform Manifold Approximation and Projection (UMAP) is a non-linear dimensionality reduction technique that aims to preserve both the local and global structure of high-dimensional data in a lower-dimensional representation.

% \subsubsection{Constructing the k-Nearest Neighbor Graph}

% UMAP begins by constructing a weighted k-nearest neighbor (k-NN) graph from the high-dimensional data. For a given dataset \( \{x_i\} \), UMAP computes the distance \( d(x_i, x_j) \) between points \( x_i \) and \( x_j \) using a distance metric, typically Euclidean distance.

% \subsubsection{Fuzzy Simplicial Set}

% UMAP constructs a fuzzy simplicial set to capture the relationships between points. This involves calculating a membership strength \( \mu_{ij} \) for each edge in the k-NN graph, indicating the probability that point \( x_i \) belongs to the neighborhood of point \( x_j \).

% \[
% \mu_{ij} = \exp\left(-\frac{d(x_i, x_j)^2 - \rho_i}{\sigma_i}\right)
% \]

% where:
% - \( d(x_i, x_j) \) is the distance between points \( x_i \) and \( x_j \),
% - \( \rho_i \) is the distance to the nearest neighbor of \( x_i \),
% - \( \sigma_i \) is a normalization factor ensuring that the local neighborhood is appropriately scaled.

% \subsubsection{Cross-Entropy Minimization}

% UMAP finds a low-dimensional embedding \( \{y_i\} \) that preserves the fuzzy topological structure of the high-dimensional data by minimizing the cross-entropy between the fuzzy simplicial set representations in the high-dimensional and low-dimensional spaces.

% The objective function for this optimization is:

% \[
% C = \sum_{(i,j)} \left[ \mu_{ij} \log \left(\frac{\mu_{ij}}{\nu_{ij}}\right) + (1 - \mu_{ij}) \log \left(\frac{1 - \mu_{ij}}{1 - \nu_{ij}}\right) \right]
% \]

% where:
% - \( \mu_{ij} \) is the membership strength in the high-dimensional space,
% - \( \nu_{ij} \) is the membership strength in the low-dimensional space, computed as:

% \[
% \nu_{ij} = \left(1 + a \cdot \| y_i - y_j \|_2^{2b} \right)^{-1}
% \]

% The parameters \( a \) and \( b \) are determined through a nonlinear optimization to ensure the low-dimensional distances are as similar as possible to the high-dimensional distances.

% \subsubsection{Optimization}

% The optimization is typically performed using stochastic gradient descent (SGD) to iteratively adjust the positions of the points \( \{y_i\} \) in the low-dimensional space to minimize the objective function \( C \).

% \subsection{HDBSCAN: Hierarchical Density-Based Spatial Clustering of Applications with Noise}

% Hierarchical Density-Based Spatial Clustering of Applications with Noise (HDBSCAN) is a clustering algorithm that extends DBSCAN by converting it into a hierarchical clustering algorithm and then extracting a flat clustering based on the stability of clusters.

% \subsubsection{Mutual Reachability Distance}

% HDBSCAN starts by defining the core distance of a point, which is the distance to its k-th nearest neighbor. For a point \( x_i \), the core distance \( d_{core}(x_i) \) is defined as:

% \[
% d_{core}(x_i) = d(x_i, x_{k-nearest}(i))
% \]

% The mutual reachability distance between two points \( x_i \) and \( x_j \) is then defined as:

% \[
% d_{mreach}(x_i, x_j) = \max\{d_{core}(x_i), d_{core}(x_j), d(x_i, x_j)\}
% \]

% \subsubsection{Constructing the Mutual Reachability Graph}

% Using the mutual reachability distance, HDBSCAN constructs a complete graph where each point is connected to every other point with edges weighted by \( d_{mreach}(x_i, x_j) \).

% \subsubsection{Minimum Spanning Tree}

% HDBSCAN constructs a minimum spanning tree (MST) from the mutual reachability graph. The MST is a subset of the edges that connects all the vertices without any cycles and with the minimum possible total edge weight.

% \subsubsection{Hierarchical Clustering}

% The MST is used to perform hierarchical clustering. HDBSCAN builds a hierarchy of clusters by progressively removing the longest edge in the MST and forming new clusters. This results in a dendrogram, which is a tree diagram that shows the arrangement of the clusters formed at each level.

% \subsubsection{Condensed Tree Representation}

% The dendrogram is then condensed into a more compact representation called the condensed tree. This is done by summarizing the hierarchical structure into a set of clusters with associated stability scores. The stability of a cluster \( C \) is defined as the sum of the excess of the points in the cluster over the minimum cluster size threshold:

% \[
% \text{stability}(C) = \sum_{x_i \in C} (\lambda_{birth}(C) - \lambda_{death}(C))
% \]

% where \( \lambda_{birth}(C) \) and \( \lambda_{death}(C) \) are the lambda values (inverse of mutual reachability distance) at which the cluster \( C \) appears and disappears in the hierarchy, respectively.

% \subsubsection{Extracting Flat Clustering}

% Finally, HDBSCAN extracts a flat clustering from the condensed tree by selecting the most stable clusters. Points that do not belong to any stable cluster are classified as noise.

% \subsection{c-TF-IDF: Class-based Term Frequency-Inverse Document Frequency}

% Class-based Term Frequency-Inverse Document Frequency (c-TF-IDF) is an adaptation of the traditional TF-IDF weighting scheme, tailored for identifying important terms within specific classes or clusters in a dataset.

% \subsubsection{Term Frequency (TF)}

% The term frequency measures how often a term \( t \) appears in a document or a class. For a given term \( t \) in a class \( c \), the term frequency \( \text{TF}(t, c) \) is defined as:

% \[
% \text{TF}(t, c) = \frac{f(t, c)}{N_c}
% \]

% where:
% - \( f(t, c) \) is the raw count of term \( t \) in class \( c \),
% - \( N_c \) is the total number of terms in class \( c \).

% \subsubsection{Document Frequency (DF)}

% The document frequency measures how many documents in the entire corpus contain the term \( t \). For a given term \( t \), the document frequency \( \text{DF}(t) \) is defined as:

% \[
% \text{DF}(t) = |\{d \mid t \in d\}|
% \]

% where:
% - \( |\{d \mid t \in d\}| \) is the number of documents containing term \( t \).

% \subsubsection{Class Inverse Document Frequency (c-IDF)}

% The class-based inverse document frequency adjusts the traditional IDF to focus on classes instead of individual documents. For a given term \( t \) in a class \( c \), the class inverse document frequency \( \text{c-IDF}(t, c) \) is defined as:

% \[
% \text{c-IDF}(t, c) = \log\left(\frac{|C|}{|\{c \mid t \in c\}|}\right)
% \]

% where:
% - \(|C|\) is the total number of classes,
% - \(|\{c \mid t \in c\}|\) is the number of classes containing term \( t \).

% \subsubsection{c-TF-IDF Calculation}

% Combining the term frequency and class inverse document frequency, the c-TF-IDF for a term \( t \) in class \( c \) is computed as:

% \[
% \text{c-TF-IDF}(t, c) = \text{TF}(t, c) \cdot \text{c-IDF}(t, c)
% \]

% Substituting the definitions of TF and c-IDF, we get:

% \[
% \text{c-TF-IDF}(t, c) = \frac{f(t, c)}{N_c} \cdot \log\left(\frac{|C|}{|\{c \mid t \in c\}|}\right)
% \]

% \subsection{Summary}

% SBERT modifies the original BERT architecture to efficiently produce sentence embeddings suitable for various downstream tasks. UMAP is a powerful dimensionality reduction technique that constructs a k-nearest neighbor graph from high-dimensional data, converts it into a fuzzy simplicial set, and optimizes a low-dimensional representation by minimizing cross-entropy. HDBSCAN extends DBSCAN by creating a hierarchical clustering structure using the mutual reachability distance and extracting the most stable clusters. Class-based Term Frequency-Inverse Document Frequency (c-TF-IDF) is an effective method for identifying important terms within specific classes or clusters. By adjusting the traditional TF-IDF to focus on class-level term importance, c-TF-IDF helps to highlight terms that are significant within particular groups of documents, making it particularly useful in topic modeling and text classification.


==> math_metrics.tex <==
\section*{Definition}





\section*{Mathematical Formula for \( C_V \) Coherence}



==> stats.tex <==
\chapter{Statistical Inferences }

\section{Statistical Test Descriptions}

\subsection{ANOVA (Analysis of Variance)}
ANOVA is a statistical method used to compare the means of three or more samples to understand if at least one of the sample means is significantly different from the others. It helps in determining whether the observed differences are statistically significant or if they occurred by chance.

\subsection{Paired t-test}
A paired t-test is used to compare two related samples, such as the same group of subjects under different conditions, to determine whether there is a statistically significant difference between their means. It is useful when the data points are dependent, such as before-and-after measurements.

\subsection{Wilcoxon Signed-Rank Test}
The Wilcoxon signed-rank test is a non-parametric alternative to the paired t-test. It compares two related samples to assess whether their population mean ranks differ. This test does not assume normal distribution of the differences and is useful for ordinal data or non-normal distributions.

\subsection{Pearson Correlation Coefficient}
The Pearson correlation coefficient measures the strength and direction of the linear relationship between two variables. It ranges from -1 to 1, where -1 indicates a perfect negative correlation, 0 indicates no correlation, and 1 indicates a perfect positive correlation.

\subsection{Tukey's Honest Significant Difference (HSD) Test}
Tukey's HSD test is a post-hoc analysis used after an ANOVA to determine which specific group means are different. It controls the Type I error rate and provides confidence intervals for the differences between means.



\section{Analysis of Number of Topics}



\subsection{ANOVA}
\begin{itemize}
    \item Sum of Squares (Model): 12014.56
    \item Sum of Squares (Residual): 2898.25
    \item F-value: 68.74
    \item p-value: $1.2 \times 10^{-11}$
\end{itemize}

The ANOVA results indicate a significant difference in the number of topics between the models (p < 0.05).

\subsection{Paired t-tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item t-statistic: 1.309
        \item p-value: 0.219
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -8.199
        \item p-value: $6.3 \times 10^{-6}$
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -7.850
        \item p-value: $8.1 \times 10^{-6}$
    \end{itemize}
\end{itemize}

The paired t-tests show significant differences between LDA and BERTopic, and between NMF and BERTopic (p < 0.05). There is no significant difference between LDA and NMF.

\subsection{Wilcoxon Signed-Rank Tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item statistic: 20.0
        \item p-value: 0.317
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
\end{itemize}

The Wilcoxon signed-rank tests confirm the significant differences between LDA and BERTopic, and between NMF and BERTopic. No significant difference is found between LDA and NMF.

\subsection{Correlation Analysis}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.821
        \item p-value: 0.001
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.521
        \item p-value: 0.081
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.511
        \item p-value: 0.087
    \end{itemize}
\end{itemize}

There is a significant positive correlation between LDA and NMF (p < 0.05). No significant correlation is found between LDA and BERTopic or between NMF and BERTopic.

\subsection{Post-hoc Tests (Tukey's HSD)}
The Tukey HSD results confirm the significant differences identified in the paired t-tests and Wilcoxon tests. Specific pairs of models show significant differences, particularly between LDA and the other models.

\subsection{Summary of Findings}
\begin{itemize}
    \item \textbf{BERTopic} consistently identifies a higher number of topics compared to LDA and NMF.
    \item Statistical tests (ANOVA, t-tests, Wilcoxon tests) indicate significant differences between BERTopic and the other models.
    \item LDA and NMF do not show significant differences in the number of topics.
    \item Correlation analysis shows a strong positive relationship between LDA and NMF in terms of the number of topics.
\end{itemize}

These findings suggest that BERTopic is more sensitive in identifying a higher number of topics within the datasets, providing more granular insights. LDA and NMF, while similar in the number of topics identified, are significantly outperformed by BERTopic in this regard.







\section{Analysis of Topic Coherence}



\subsection{ANOVA}
\begin{itemize}
    \item Sum of Squares (Model): 0.226
    \item Sum of Squares (Residual): 0.176
    \item F-value: 21.246
    \item p-value: 0.000001
\end{itemize}

The ANOVA results indicate a significant difference in topic coherence between the models (p $ < $ 0.05).

\subsection{Paired t-tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item t-statistic: -9.050
        \item p-value: 1.99e-06
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -7.837
        \item p-value: 7.94e-06
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item t-statistic: 1.311
        \item p-value: 0.216
    \end{itemize}
\end{itemize}

The paired t-tests show significant differences between LDA and NMF, and between LDA and BERTopic (p < 0.05). There is no significant difference between NMF and BERTopic.

\subsection{Wilcoxon Signed-Rank Tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.000488
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.000488
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item statistic: 24.0
        \item p-value: 0.266
    \end{itemize}
\end{itemize}

The Wilcoxon signed-rank tests confirm the significant differences between LDA and NMF, and between LDA and BERTopic. No significant difference is found between NMF and BERTopic.

\subsection{Correlation Analysis}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.783
        \item p-value: 0.0026
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.178
        \item p-value: 0.579
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.311
        \item p-value: 0.326
    \end{itemize}
\end{itemize}

There is a significant positive correlation between LDA and NMF (p < 0.05). No significant correlation is found between LDA and BERTopic or between NMF and BERTopic.

\subsection{Post-hoc Tests (Tukey's HSD)}
The Tukey HSD results confirm the significant differences identified in the paired t-tests and Wilcoxon tests. Specific pairs of models show significant differences, particularly between LDA and the other models.

\subsection{Summary of Findings}
\begin{itemize}
    \item \textbf{LDA} consistently has lower topic coherence compared to NMF and BERTopic.
    \item \textbf{NMF} generally has higher coherence scores than LDA but shows no significant difference compared to BERTopic.
    \item \textbf{BERTopic} has similar coherence scores to NMF and significantly higher than LDA.
    \item Statistical tests (ANOVA, t-tests, Wilcoxon tests) consistently indicate significant differences between LDA and the other models.
    \item Correlation analysis shows a strong positive relationship between LDA and NMF coherence scores.
\end{itemize}

These findings suggest that while NMF and BERTopic both provide high-quality topics in terms of coherence, BERTopic does not significantly outperform NMF in this metric. LDA, however, is consistently outperformed by both NMF and BERTopic.



\section{Analysis of Topic Diversity}

\subsection{Descriptive Statistics}


\subsection{ANOVA}
\begin{itemize}
    \item Sum of Squares (Model): 0.643
    \item Sum of Squares (Residual): 0.041
    \item F-value: 257.26
    \item p-value: $2.2 \times 10^{-18}$
\end{itemize}

The ANOVA results indicate a significant difference in topic diversity between the models (p < 0.05).

\subsection{Paired t-tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item t-statistic: -7.376
        \item p-value: $1.8 \times 10^{-5}$
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -14.248
        \item p-value: $3.4 \times 10^{-8}$
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -8.537
        \item p-value: $4.9 \times 10^{-6}$
    \end{itemize}
\end{itemize}

The paired t-tests show significant differences between all pairs of models (p < 0.05).

\subsection{Wilcoxon Signed-Rank Tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
\end{itemize}

The Wilcoxon signed-rank tests confirm the significant differences between all pairs of models.

\subsection{Correlation Analysis}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.748
        \item p-value: 0.005
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.636
        \item p-value: 0.028
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.606
        \item p-value: 0.038
    \end{itemize}
\end{itemize}

There are significant positive correlations between all pairs of models (p < 0.05).

\subsection{Post-hoc Tests (Tukey's HSD)}
The Tukey HSD results confirm the significant differences identified in the paired t-tests and Wilcoxon tests. Specific pairs of models show significant differences.

\subsection{Summary of Findings}
\begin{itemize}
    \item \textbf{BERTopic} consistently shows the highest topic diversity compared to LDA and NMF.
    \item Statistical tests (ANOVA, t-tests, Wilcoxon tests) indicate significant differences between all pairs of models.
    \item Correlation analysis shows strong positive relationships between the topic diversity scores of all models.
\end{itemize}

These findings suggest that BERTopic provides the highest topic diversity, indicating that it generates more unique and varied topics compared to LDA and NMF. All models show significant differences in topic diversity, with BERTopic performing the best.


\section{Analysis of KL-Divergence}



\subsection{ANOVA}
\begin{itemize}
    \item Sum of Squares (Model): 519.79
    \item Sum of Squares (Residual): 20.68
    \item F-value: 415.13
    \item p-value: $1.1 \times 10^{-19}$
\end{itemize}

The ANOVA results indicate a significant difference in KL-Divergence between the models (p < 0.05).

\subsection{Paired t-tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item t-statistic: -25.642
        \item p-value: $1.4 \times 10^{-11}$
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item t-statistic: 6.245
        \item p-value: $4.1 \times 10^{-5}$
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item t-statistic: 20.921
        \item p-value: $6.3 \times 10^{-11}$
    \end{itemize}
\end{itemize}

The paired t-tests show significant differences between all pairs of models (p < 0.05).

\subsection{Wilcoxon Signed-Rank Tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item statistic: 66.0
        \item p-value: 0.00098
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
\end{itemize}

The Wilcoxon signed-rank tests confirm the significant differences between all pairs of models.

\subsection{Correlation Analysis}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.542
        \item p-value: 0.070
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.681
        \item p-value: 0.015
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.592
        \item p-value: 0.042
    \end{itemize}
\end{itemize}

There are significant positive correlations between LDA and BERTopic, and between NMF and BERTopic (p < 0.05). No significant correlation is found between LDA and NMF.

\subsection{Post-hoc Tests (Tukey's HSD)}
The Tukey HSD results confirm the significant differences identified in the paired t-tests and Wilcoxon tests. Specific pairs of models show significant differences.

\subsection{Summary of Findings}
\begin{itemize}
    \item \textbf{NMF} consistently shows the highest KL-Divergence compared to LDA and BERTopic.
    \item Statistical tests (ANOVA, t-tests, Wilcoxon tests) indicate significant differences between all pairs of models.
    \item Correlation analysis shows strong positive relationships between the KL-Divergence scores of LDA and BERTopic, and between NMF and BERTopic.
\end{itemize}

These findings suggest that NMF provides the highest KL-Divergence, indicating a larger divergence from the actual topic distributions compared to LDA and BERTopic. All models show significant differences in KL-Divergence, with NMF performing the worst in this regard.


\section{Analysis of Perplexity}



\subsection{ANOVA}
\begin{itemize}
    \item Sum of Squares (Model): 762524.03
    \item Sum of Squares (Residual): 29807.18
    \item F-value: 430.61
    \item p-value: $3.1 \times 10^{-20}$
\end{itemize}

The ANOVA results indicate a significant difference in Perplexity between the models (p < 0.05).

\subsection{Paired t-tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item t-statistic: -7.402
        \item p-value: $1.7 \times 10^{-5}$
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -57.536
        \item p-value: $3.3 \times 10^{-14}$
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item t-statistic: 7.256
        \item p-value: $2.0 \times 10^{-5}$
    \end{itemize}
\end{itemize}

The paired t-tests show significant differences between all pairs of models (p < 0.05).

\subsection{Wilcoxon Signed-Rank Tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
\end{itemize}

The Wilcoxon signed-rank tests confirm the significant differences between all pairs of models.

\subsection{Correlation Analysis}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item Pearson correlation coefficient: -0.632
        \item p-value: 0.030
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: -0.803
        \item p-value: 0.002
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.703
        \item p-value: 0.012
    \end{itemize}
\end{itemize}

There are significant negative correlations between LDA and NMF, and between LDA and BERTopic (p < 0.05). A significant positive correlation is found between NMF and BERTopic.

\subsection{Post-hoc Tests (Tukey's HSD)}
The Tukey HSD results confirm the significant differences identified in the paired t-tests and Wilcoxon tests. Specific pairs of models show significant differences.

\subsection{Summary of Findings}
\begin{itemize}
    \item \textbf{NMF} consistently shows the highest Perplexity compared to LDA and BERTopic.
    \item Statistical tests (ANOVA, t-tests, Wilcoxon tests) indicate significant differences between all pairs of models.
    \item Correlation analysis shows strong negative relationships between the Perplexity scores of LDA and NMF, and between LDA and BERTopic. A strong positive relationship is found between NMF and BERTopic.
\end{itemize}

These findings suggest that NMF provides the highest Perplexity, indicating a poorer predictive performance compared to LDA and BERTopic. All models show significant differences in Perplexity, with NMF performing the worst in this regard.


\section{Analysis of Execution Time}

\subsection{Descriptive Statistics}


\subsection{ANOVA}
\begin{itemize}
    \item Sum of Squares (Model): 8305642.36
    \item Sum of Squares (Residual): 330025.79
    \item F-value: 151.66
    \item p-value: $1.2 \times 10^{-18}$
\end{itemize}

The ANOVA results indicate a significant difference in execution time between the models (p < 0.05).

\subsection{Paired t-tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item t-statistic: 4.248
        \item p-value: $0.0016$
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item t-statistic: 0.105
        \item p-value: $0.918$
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item t-statistic: -7.024
        \item p-value: $3.7 \times 10^{-5}$
    \end{itemize}
\end{itemize}

The paired t-tests show significant differences between LDA and NMF, and between NMF and BERTopic (p < 0.05). There is no significant difference between LDA and BERTopic.

\subsection{Wilcoxon Signed-Rank Tests}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00098
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item statistic: 37.0
        \item p-value: 0.793
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item statistic: 0.0
        \item p-value: 0.00049
    \end{itemize}
\end{itemize}

The Wilcoxon signed-rank tests confirm the significant differences between LDA and NMF, and between NMF and BERTopic. No significant difference is found between LDA and BERTopic.

\subsection{Correlation Analysis}
\begin{itemize}
    \item \textbf{LDA vs NMF}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.554
        \item p-value: 0.061
    \end{itemize}
    \item \textbf{LDA vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.960
        \item p-value: $4.8 \times 10^{-7}$
    \end{itemize}
    \item \textbf{NMF vs BERTopic}:
    \begin{itemize}
        \item Pearson correlation coefficient: 0.521
        \item p-value: 0.080
    \end{itemize}
\end{itemize}

There is a significant positive correlation between LDA and BERTopic (p < 0.05). No significant correlation is found between LDA and NMF, or between NMF and BERTopic.

\subsection{Post-hoc Tests (Tukey's HSD)}
The Tukey HSD results confirm the significant differences identified in the paired t-tests and Wilcoxon tests. Specific pairs of models show significant differences.

\subsection{Summary of Findings}
\begin{itemize}
    \item \textbf{NMF} consistently shows the lowest execution time compared to LDA and BERTopic.
    \item Statistical tests (ANOVA, t-tests, Wilcoxon tests) indicate significant differences between LDA and NMF, and between NMF and BERTopic.
    \item No significant difference in execution time is found between LDA and BERTopic.
    \item Correlation analysis shows a strong positive relationship between the execution times of LDA and BERTopic.
\end{itemize}

These findings suggest that NMF is the most computationally efficient model, requiring significantly less execution time compared to LDA and BERTopic. LDA and BERTopic show similar execution times, with no significant difference between them.


\section{Conclusion}

This analysis compared three topic modeling methods (LDA, NMF, and BERTopic) across various metrics: Number of Topics, Topic Coherence, Topic Diversity, KL-Divergence, Perplexity, and Execution Time. The following summarizes the findings for each model based on the statistical tests conducted:

\subsection{LDA (Latent Dirichlet Allocation)}
\begin{itemize}
    \item \textbf{Number of Topics}: LDA identified a moderate number of topics, with significant differences compared to BERTopic but not NMF.
    \item \textbf{Topic Coherence}: LDA showed the lowest coherence scores, significantly lower than both NMF and BERTopic.
    \item \textbf{Topic Diversity}: LDA exhibited lower diversity compared to NMF and BERTopic, with significant differences between all pairs.
    \item \textbf{KL-Divergence}: LDA had significantly lower KL-Divergence than NMF, indicating better alignment with actual topic distributions, but higher than BERTopic.
    \item \textbf{Perplexity}: LDA had lower perplexity than NMF, indicating better predictive performance, but higher than BERTopic.
    \item \textbf{Execution Time}: LDA's execution time was significantly longer than NMF but similar to BERTopic.
\end{itemize}

\subsection{NMF (Non-negative Matrix Factorization)}
\begin{itemize}
    \item \textbf{Number of Topics}: NMF identified fewer topics than LDA and significantly fewer than BERTopic.
    \item \textbf{Topic Coherence}: NMF had higher coherence scores than LDA and was comparable to BERTopic.
    \item \textbf{Topic Diversity}: NMF showed higher diversity than LDA but was significantly lower than BERTopic.
    \item \textbf{KL-Divergence}: NMF had the highest KL-Divergence, indicating the poorest alignment with actual topic distributions.
    \item \textbf{Perplexity}: NMF exhibited the highest perplexity, indicating the worst predictive performance.
    \item \textbf{Execution Time}: NMF was the most computationally efficient, with significantly lower execution times than both LDA and BERTopic.
\end{itemize}

\subsection{BERTopic}
\begin{itemize}
    \item \textbf{Number of Topics}: BERTopic identified the highest number of topics, significantly more than both LDA and NMF.
    \item \textbf{Topic Coherence}: BERTopic had the highest coherence scores, significantly higher than LDA and comparable to NMF.
    \item \textbf{Topic Diversity}: BERTopic showed the highest diversity, significantly higher than both LDA and NMF.
    \item \textbf{KL-Divergence}: BERTopic had the lowest KL-Divergence, indicating the best alignment with actual topic distributions.
    \item \textbf{Perplexity}: BERTopic exhibited the lowest perplexity, indicating the best predictive performance.
    \item \textbf{Execution Time}: BERTopic's execution time was significantly longer than NMF but similar to LDA.
\end{itemize}

\subsection{Overall Comparison}
\begin{itemize}
    \item \textbf{Quality of Topics}: BERTopic generally produced the highest quality topics in terms of coherence, diversity, and alignment with actual topic distributions.
    \item \textbf{Predictive Performance}: BERTopic showed the best predictive performance as indicated by the lowest perplexity.
    \item \textbf{Computational Efficiency}: NMF was the most computationally efficient method, requiring significantly less execution time.
    \item \textbf{Topic Quantity}: BERTopic identified the most topics, providing more granular insights, while NMF identified the fewest.
\end{itemize}

In conclusion, BERTopic outperforms LDA and NMF in most quality metrics, albeit with higher computational costs compared to NMF. NMF, while computationally efficient, lags in topic quality metrics. LDA offers a middle ground but is generally outperformed by BERTopic in terms of topic quality and predictive performance.


==> uw-ethesis-frontpgs.tex <==
% T I T L E   P A G E
% -------------------
% Last updated August 24, 2023, by IST-Client Services
% The title page is counted as page `i' but we need to suppress the
% page number. Also, we don't want any headers or footers.
\pagestyle{empty}
\pagenumbering{roman}

% The contents of the title page are specified in the "titlepage"
% environment.
\begin{titlepage}
        \begin{center}
        \vspace*{1.0cm}

        \Huge
        {\bf A Comparison of Unsupervised Topic Modelling Techniques for Qualitative Data Analysis of Online Communities }

        \vspace*{1.0cm}

        \normalsize
        by \\

        \vspace*{1.0cm}

        \Large
        Amandeep Kaur\\

        \vspace*{3.0cm}

        \normalsize
        A thesis \\
        presented to the University of Waterloo \\ 
        in fulfillment of the \\
        thesis requirement for the degree of \\
        Master of Mathematics \\
        in \\
        Computer Science \\

        \vspace*{1.0cm}

        Waterloo, Ontario, Canada, 2024 \\

        \vspace*{0.5cm}

                \copyright\ Amandeep Kaur 2024 \\
        \end{center}
\end{titlepage}

% The rest of the front pages should contain no headers and be numbered using Roman numerals starting with `ii'
\pagestyle{plain}
\setcounter{page}{2}

\cleardoublepage % Ends the current page and causes all figures and tables that have so far appeared in the input to be printed.
% In a two-sided printing style, it also makes the next page a right-hand (odd-numbered) page, producing a blank page if necessary.
\phantomsection    % allows hyperref to link to the correct page
 
% E X A M I N I N G   C O M M I T T E E (Required for Ph.D. theses only)
% Remove or comment out the lines below to remove this page
% \addcontentsline{toc}{chapter}{Examining Committee}
% \begin{center}\textbf{Examining Committee Membership}\end{center}
%   \noindent
% The following served on the Examining Committee for this thesis. The decision of the Examining Committee is by majority vote.
%   \bigskip
  

  
%   \noindent
% \begin{tabbing}
% Internal-External Member: \=  \kill % using longest text to define tab length
% Supervisor(s): \> Prof. James R. Wallace \\
% \> Associate Professor \\
% \> School of Public Health Sciences \\
% \>David R. Cheriton Schoool of Computer Science \\

% \> University of Waterloo \\

% \end{tabbing}
%   \bigskip
  
%   \noindent
%   \begin{tabbing}
% Internal-External Member: \=  \kill % using longest text to define tab length
% Internal Member: \> Prof. Jesse Hoey\\
% \> Professor
% \\
% \>David R. Cheriton Schoool of Computer Science \\
% \>University of Waterloo \\
% \end{tabbing}
%   \bigskip
  
%   \noindent
% \begin{tabbing}
% Internal-External Member: \=  \kill % using longest text to define tab length
% Internal Member: \> Prof. Jian Zhao \\
% \> Assistant Professor \\
% \>David R. Cheriton Schoool of Computer Science \\
% \>University of Waterloo \\
% \end{tabbing}
%   \bigskip
  


\cleardoublepage
\phantomsection    % allows hyperref to link to the correct page

% D E C L A R A T I O N   P A G E
% -------------------------------
  % The following is a sample Declaration Page as provided by the GSPA
  % December 13th, 2006.  It is designed for an electronic thesis.
 \addcontentsline{toc}{chapter}{Author's Declaration}
 \begin{center}\textbf{Author's Declaration}\end{center}

 % Author's Declaration Option ONE - line 118:  
 \noindent
I hereby declare that I am the sole author of this thesis. This is a true copy of the thesis, including any required final revisions, as accepted by my examiners.
  % Author's Declaration Option TWO - line 121. Updated August 21st, 2023. Use the following declaration text if appropriate by removing the percent character and space at the beginning of line 121, and add a percent symbol and space at line 118 to change Author's Declaration Option ONE to a remark that is not printed.
 \noindent  
% This thesis consists of material all of which I authored or co-authored: see Statement of Contributions included in the thesis. This is a true copy of the thesis, including any required final revisions, as accepted by my examiners.
  \bigskip
  
  \noindent
I understand that my thesis may be made electronically available to the public.

\cleardoublepage
\phantomsection    % allows hyperref to link to the correct page

% A B S T R A C T
% ---------------
\addcontentsline{toc}{chapter}{Abstract}
\begin{center}\textbf{Abstract}\end{center}

Social media constitutes a rich and influential source of information for qualitative researchers. However, its vast volume and diversity present significant challenges, which can be assisted by computational techniques like topic modelling. But qualitative researchers often struggle to use computational techniques due to a lack of programming expertise and concerns about maintaining the nuanced aspects of their research, such as contextual understanding, subjective interpretations,  and ethical considerations of their data. To address this issue, this thesis explores the integration of BERTopic, an advanced Large Language Model (LLM)-based method, into the Computational Thematic Analysis (CTA) Toolkit to support qualitative data analysis of social media. We conducted interviews and hands-on evaluations in which qualitative researchers compared topics from three modeling techniques --- LDA, NMF and BERTopic. Participants prioritized topic relevance, logical organization, and the capacity to reveal unexpected relationships within the data, valuing detailed, coherent clusters for deeper understanding and actionable insights. BERTopic was favored by 8/12 participants for its ability to uncover hidden connections. These findings underscore the transformative potential of LLM-based tools in providing deeper, more nuanced insights for qualitative analysis of social media data.

\cleardoublepage
\phantomsection    % allows hyperref to link to the correct page

% A C K N O W L E D G E M E N T S
% -------------------------------
\addcontentsline{toc}{chapter}{Acknowledgements}
\begin{center}\textbf{Acknowledgements}\end{center}
\begin{center}
    \textbf{Territorial Acknowledgements}
\end{center}

During my Master’s research, I spent most of my time living and working in the traditional territory of the Attawandaron (also known as Neutral), Anishinaabe and Haudenosaunee peoples. My rental home (Columbia Lake Village) and the University of Waterloo are situated on the Haldimand Tract, the land promised to the Six Nations in 1784 that includes six miles on each side of the Grand River.
 \\
 \begin{center}
    \textbf{Funding Acknowledgements}
\end{center}

 

My gratitude to all sources of my funding including:
\begin{itemize}
    \item Graduate Teaching Assistant Positions at the University of Waterloo, David R. Cheriton School of Computer Science 
    \item Graduate Research Assistant Positions at the University of Waterloo, David R. Cheriton School of Computer Science 
\item International Master’s Award of Excellence, University of Waterloo, David R. Cheriton School of Computer Science 
\item Natural Sciences and Engineering Research Council of Canada (NSERC) Discovery Grants 
\item MITACS Globalink Graduate Fellowship 



\end{itemize}


 
\cleardoublepage
\phantomsection    % allows hyperref to link to the correct page

% D E D I C A T I O N
% % -------------------
% \addcontentsline{toc}{chapter}{Acknowledgements}
\begin{center}\textbf{Personal Acknowledgements}\end{center}

To Professor James R. Wallace, my supervisor, whose support, and guidance have been invaluable throughout my thesis journey. Your unwavering support at every stage of this journey, from brainstorming initial ideas to refining the final process, has provided me with the confidence and resources necessary to succeed. I am deeply grateful for the opportunity you provided me and for the mentorship you offered.

To Professor Jesse Hoey and Professor Jian Zhao, thank you for taking the time to read my thesis and for offering your insights and guidance on how to improve my work.

To Professor Robin Cohen, Professor Paulo Alencar, and Professor Jian Zhao for teaching graduate-level courses in such a captivating and enjoyable manner. Your classes were not only valuable but also enhanced my presentation skills, making interactions with classmates something I eagerly anticipated.  

To my grandmothers, Mrs. Harbans Kaur and Mrs. Paramjit Kaur, and my late grandfathers, Er. Lal Singh and Mr. Gurdev Singh, thank you for your unwavering encouragement and belief in my dream of pursuing a master's degree abroad. In times of difficulty, your support and nurturing presence gave me the strength to remain hopeful and resilient. 

To my parents, Mrs. Paramjeet Kaur and Mr. Baljinder Singh, your constant support has been the bedrock of my success. Your love and encouragement have sustained me through every challenge. Thank you for always reminding me of my worth and potential, and for being my guiding lights along this journey. Also, thanks to my sibling Mehardeep Singh for always believing in me! 

To my uncle, Dr. Kanwaljit Singh, and aunt, Er. Balbir Kaur, I am deeply grateful for your advice and guidance throughout my academic journey. Your unwavering belief in the power of perseverance and your encouragement to keep pushing forward, even in the face of obstacles, have been a source of strength and inspiration. 


To all my dear friends from the Computer Science, Engineering, Environment, Science and Health departments, Games Institute and CSGSA fellows, your companionship made my time on campus memorable and fulfilling.

To my labmates, Ansh Sharma and Robert Gauthier, for always being there to discuss research and share life’s experiences. And to the CS graduate office and CSCF, thank you for your support throughout this journey.

\cleardoublepage
\phantomsection    % allows hyperref to link to the correct page

% T A B L E   O F   C O N T E N T S
% ---------------------------------
\renewcommand\contentsname{Table of Contents}
\tableofcontents
\cleardoublepage
\phantomsection    % allows hyperref to link to the correct page

% L I S T   O F   F I G U R E S
% -----------------------------
\addcontentsline{toc}{chapter}{List of Figures}
\listoffigures
\cleardoublepage
\phantomsection		% allows hyperref to link to the correct page

% L I S T   O F   T A B L E S
% ---------------------------
\addcontentsline{toc}{chapter}{List of Tables}
\listoftables
\cleardoublepage
\phantomsection		% allows hyperref to link to the correct page

% L I S T   O F   A B B R E V I A T I O N S
% ---------------------------
\renewcommand*{\abbreviationsname}{List of Abbreviations}
\printglossary[type=abbreviations]
\cleardoublepage
\phantomsection		% allows hyperref to link to the correct page

% L I S T   O F   S Y M B O L S
% ---------------------------
\printglossary[type=symbols]
\cleardoublepage
\phantomsection		% allows hyperref to link to the correct page


% Change page numbering back to Arabic numerals
\pagenumbering{arabic}


